Quantum Meets Fine-grained Complexity: Sublinear Time Quantum Algorithms for String Problems

Longest common substring (LCS), longest palindrome substring (LPS), and Ulam distance (UL) are three fundamental string problems that can be classically solved in near linear time. In this work, we present sublinear time quantum algorithms for these problems along with quantum lower bounds. Our results shed light on a very surprising fact: Although the classic solutions for LCS and LPS are almost identical (via suffix trees), their quantum computational complexities are different. While we give an exact $\tilde O(\sqrt{n})$ time algorithm for LPS, we prove that LCS needs at least time $\tilde \Omega(n^{2/3})$ even for 0/1 strings.

==> figs/old/f1.tex <==
\begin{figure}[!htbp]
	\centering
	
	
	
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
	
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,306); %set diagram left start at 0, and has height of 306
	
	%Shape: Rectangle [id:dp3556060999220616] 
	\draw   (52,100) -- (607,100) -- (607,131) -- (52,131) -- cycle ;
	%Shape: Rectangle [id:dp06231417991804866] 
	\draw  [fill={rgb, 255:red, 255; green, 210; blue, 132 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (219.5,104) -- (420,104) -- (420,127) -- (219.5,127) -- cycle ;
	%Shape: Rectangle [id:dp2722965559510331] 
	\draw   (52,160) -- (607,160) -- (607,191) -- (52,191) -- cycle ;
	%Shape: Rectangle [id:dp652490843803089] 
	\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (258.5,164) -- (510.5,164) -- (510.5,187) -- (258.5,187) -- cycle ;
	%Shape: Rectangle [id:dp6481666444378198] 
	\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.32 ][dash pattern={on 0.84pt off 2.51pt}] (179.5,64) -- (468.5,64) -- (468.5,87) -- (179.5,87) -- cycle ;
	%Shape: Rectangle [id:dp5402617564265502] 
	\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (249.5,208) -- (591.5,208) -- (591.5,231) -- (249.5,231) -- cycle ;
	%Shape: Rectangle [id:dp47493868229303815] 
	\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.4 ][dash pattern={on 0.84pt off 2.51pt}] (159.5,28) -- (448.5,28) -- (448.5,51) -- (159.5,51) -- cycle ;
	%Shape: Rectangle [id:dp7711694349164948] 
	\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.4 ][dash pattern={on 0.84pt off 2.51pt}] (229.5,238) -- (518.5,238) -- (518.5,261) -- (229.5,261) -- cycle ;
	%Straight Lines [id:da4301971719945532] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (179.5,87) -- (249.5,231) ;
	%Straight Lines [id:da601947917319118] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (179.5,87) -- (179.5,19) ;
	%Straight Lines [id:da2813252871480405] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (468.5,87) -- (468.5,19) ;
	%Straight Lines [id:da409858789619455] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (249.5,277) -- (249.5,209) ;
	%Straight Lines [id:da3241817701092482] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (591.5,276) -- (591.5,208) ;
	
	% Text Node
	\draw (27,107.4) node [anchor=north west][inner sep=0.75pt]    {$A$};
	% Text Node
	\draw (27,167.4) node [anchor=north west][inner sep=0.75pt]    {$B$};
	% Text Node
	\draw (317,107.4) node [anchor=north west][inner sep=0.75pt]    {$P$};
	% Text Node
	\draw (175,-0.6) node [anchor=north west][inner sep=0.75pt]    {$\alpha $};
	% Text Node
	\draw (461,-0.6) node [anchor=north west][inner sep=0.75pt]    {$\beta $};
	% Text Node
	\draw (244,278.4) node [anchor=north west][inner sep=0.75pt]    {$\alpha '$};
	% Text Node
	\draw (587,274.4) node [anchor=north west][inner sep=0.75pt]    {$\beta '$};
	
	
	\end{tikzpicture}
	

	\caption{The red intervals correspond to the longest common substring. The yellow interval is $P$ and the green interval is $S[\ell,r+|P|-']$. The blue and grey intervals are extensions of the yellow and green intervals so long as they remain $(r-\ell)$-periodic.}\label{fig:1}
\end{figure}

==> figs/old/f2.tex <==
\begin{figure}[!htbp]
	\centering
	
	
	
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
	
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,306); %set diagram left start at 0, and has height of 306
	
	%Shape: Rectangle [id:dp28043622005715463] 
	\draw   (52,100) -- (607,100) -- (607,131) -- (52,131) -- cycle ;
	%Shape: Rectangle [id:dp5129187326740472] 
	\draw  [fill={rgb, 255:red, 255; green, 210; blue, 132 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (219.5,104) -- (420,104) -- (420,127) -- (219.5,127) -- cycle ;
	%Shape: Rectangle [id:dp12301789036874666] 
	\draw   (52,160) -- (607,160) -- (607,191) -- (52,191) -- cycle ;
	%Shape: Rectangle [id:dp8287338354113372] 
	\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (258.5,164) -- (510.5,164) -- (510.5,187) -- (258.5,187) -- cycle ;
	%Shape: Rectangle [id:dp800039771753196] 
	\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.32 ][dash pattern={on 0.84pt off 2.51pt}] (179.5,64) -- (468.5,64) -- (468.5,87) -- (179.5,87) -- cycle ;
	%Shape: Rectangle [id:dp06838977775166755] 
	\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (249.5,208) -- (543.5,208) -- (543.5,231) -- (249.5,231) -- cycle ;
	%Shape: Rectangle [id:dp5107101648811607] 
	\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.4 ][dash pattern={on 0.84pt off 2.51pt}] (207.5,28) -- (506.5,28) -- (506.5,51) -- (207.5,51) -- cycle ;
	%Shape: Rectangle [id:dp3854720525307225] 
	\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.4 ][dash pattern={on 0.84pt off 2.51pt}] (287.5,237) -- (576.5,237) -- (576.5,260) -- (287.5,260) -- cycle ;
	%Straight Lines [id:da19062063883642755] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (468.5,87) -- (543.5,231) ;
	%Straight Lines [id:da13623302453706] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (179.5,87) -- (179.5,19) ;
	%Straight Lines [id:da8750939304782699] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (468.5,87) -- (468.5,19) ;
	%Straight Lines [id:da26994651928063185] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (249.5,277) -- (249.5,209) ;
	%Straight Lines [id:da10551294597035388] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (543.5,276) -- (543.5,208) ;
	
	% Text Node
	\draw (27,107.4) node [anchor=north west][inner sep=0.75pt]    {$A$};
	% Text Node
	\draw (27,167.4) node [anchor=north west][inner sep=0.75pt]    {$B$};
	% Text Node
	\draw (317,107.4) node [anchor=north west][inner sep=0.75pt]    {$P$};
	% Text Node
	\draw (175,-0.6) node [anchor=north west][inner sep=0.75pt]    {$\alpha $};
	% Text Node
	\draw (461,-0.6) node [anchor=north west][inner sep=0.75pt]    {$\beta $};
	% Text Node
	\draw (244,278.4) node [anchor=north west][inner sep=0.75pt]    {$\alpha '$};
	% Text Node
	\draw (539,274.4) node [anchor=north west][inner sep=0.75pt]    {$\beta '$};
	
	
	\end{tikzpicture}
	
	\caption{The red intervals correspond to the longest common substring. The yellow interval is $P$ and the green interval is $S[\ell,r+|P|-']$. The blue and grey intervals are extensions of the yellow and green intervals so long as they remain $(r-\ell)$-periodic.}\label{fig:2}
\end{figure}

==> figs/old/f3.tex <==
\begin{figure}[!htbp]
	\centering
	
	
	
	
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
	
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,306); %set diagram left start at 0, and has height of 306
	
	%Shape: Rectangle [id:dp5111115517803526] 
	\draw   (52,100) -- (607,100) -- (607,131) -- (52,131) -- cycle ;
	%Shape: Rectangle [id:dp6187538708036826] 
	\draw  [fill={rgb, 255:red, 255; green, 210; blue, 132 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (219.5,104) -- (420,104) -- (420,127) -- (219.5,127) -- cycle ;
	%Shape: Rectangle [id:dp741755322257067] 
	\draw   (52,160) -- (607,160) -- (607,191) -- (52,191) -- cycle ;
	%Shape: Rectangle [id:dp9864868964350268] 
	\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (258.5,164) -- (510.5,164) -- (510.5,187) -- (258.5,187) -- cycle ;
	%Shape: Rectangle [id:dp5352816322735938] 
	\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.32 ][dash pattern={on 0.84pt off 2.51pt}] (179.5,64) -- (468.5,64) -- (468.5,87) -- (179.5,87) -- cycle ;
	%Shape: Rectangle [id:dp06199639773072518] 
	\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (249.5,208) -- (543.5,208) -- (543.5,231) -- (249.5,231) -- cycle ;
	%Shape: Rectangle [id:dp10030551230571794] 
	\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.4 ][dash pattern={on 0.84pt off 2.51pt}] (207.5,28) -- (446.5,28) -- (446.5,51) -- (207.5,51) -- cycle ;
	%Straight Lines [id:da11421675549326493] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (179.5,87) -- (179.5,19) ;
	%Straight Lines [id:da8616607053184913] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (468.5,87) -- (468.5,19) ;
	%Straight Lines [id:da13847993447336493] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (249.5,277) -- (249.5,209) ;
	%Straight Lines [id:da34950919757773624] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (543.5,276) -- (543.5,208) ;
	%Shape: Rectangle [id:dp7220005061667816] 
	\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.4 ][dash pattern={on 0.84pt off 2.51pt}] (287.5,248) -- (526.5,248) -- (526.5,271) -- (287.5,271) -- cycle ;
	
	% Text Node
	\draw (27,107.4) node [anchor=north west][inner sep=0.75pt]    {$A$};
	% Text Node
	\draw (27,167.4) node [anchor=north west][inner sep=0.75pt]    {$B$};
	% Text Node
	\draw (317,107.4) node [anchor=north west][inner sep=0.75pt]    {$P$};
	% Text Node
	\draw (175,-0.6) node [anchor=north west][inner sep=0.75pt]    {$\alpha $};
	% Text Node
	\draw (461,-0.6) node [anchor=north west][inner sep=0.75pt]    {$\beta $};
	% Text Node
	\draw (244,278.4) node [anchor=north west][inner sep=0.75pt]    {$\alpha '$};
	% Text Node
	\draw (539,274.4) node [anchor=north west][inner sep=0.75pt]    {$\beta '$};
	
	
	\end{tikzpicture}
	
	
	\caption{The red intervals correspond to the longest common substring. The yellow interval is $P$ and the green interval is $S[\ell,r+|P|-']$. The blue and grey intervals are extensions of the yellow and green intervals so long as they remain $(r-\ell)$-periodic.}\label{fig:3}
\end{figure}

==> src/old files/lcs-old3.tex <==
% !TEX root = ../draft.tex
\section{Longest Common Substring}
Remember that in longest common substring, we are given two strings $A$ and $B$ of size $n$ and the goal is to find the largest string $t$ which is a substring of both $A$ and $B$. This problem can be solved in time $O(n)$ via suffix tree in the classic setting. In this section, we give upper bounds for the quantum complexity of this problem (lower bounds are discussed in Section \ref{section:lb}). We first begin by giving an algorithm for exact \textsf{LCS} that runs in time $\tilde O(n^{5/6})$ in Section \ref{sub:lcs-exact}. We then give an algorithm for approximated \textsf{LCS} that runs in time $\tilde O(n^{3/4})$ in Section \ref{sub:lcs-approximate}. 

\subsection{Quantum algorithm for exact \textsf{LCS}}\label{sub:lcs-exact}
In our algorithm, we do a binary search on the size of the solution. We denote this value by $d$. Thus, by losing an $O(\log n)$ factor in the runtime, we reduce the problem to verifying if a substring of size $d$ is shared between the two strings. Our approach is twofold; we design separate algorithms for small and large $d$.

\paragraph*{Quantum algorithm for small $d$.}
Our algorithm for small $d$ is inspired by a variant of \textit{element distinctness}. In this variant, two sets of pointers $S_A$ and $S_B$ are given and the goal is to verify if the two sets share a common element. It has been shown~\cite{ambainis2007quantum} that element distinctness can be solved in time $\tilde O(n^{2/3})$ if the number of elements in the two sets is equal to $n$. Moreover, the algorithm uses oracle queries that compare the elements. The total number of queries made to the oracle is also $\tilde O(n^{2/3})$~\cite{ambainis2007quantum}. For small $d$, we use element distinctness. Let $|\Sigma|$ be the size of the alphabet and $v:\Sigma \rightarrow [0,|\Sigma|-1]$ be a function that maps every element of the alphabet to a distinct number in range $0 \ldots |\Sigma|-1$. In other words, $v$ is a perfect hashing for the characters. We extend this definition to substrings of the two strings. For a string $t$, we define $v(t)$ as follows:

$$v(t) = \sum_{i = 1}^{|t|} v(t_i) |\Sigma|^{i-1}.$$

It follows from the definition that two strings $t_1$ and $t_2$ are equal if and only if we have $v(t_1) = v(t_2)$. From the two strings, we make two sets of numbers $S_A$ and $S_B$ each having $n-d+1$ elements. Element $i$ of set $S_A$ is a pair $(A,i)$ whose value is equal to $v(A[i,i+d-1])$ and similarly element $i$ of $S_B$ is a pair $(B,i)$ whose value is equal to $v(B[i,i+d-1])$. Note that the size of the representation for each element is $O(1)$ but comparing elements takes time $\Omega(1)$. The two sets contain elements with equal values if and only if the two strings have a common substring of size $d$. Therefore, by solving element distinctness for $S_A$ and $S_B$ we can find out if the size of the solution is at least $d$. Although element distinctness can be solved in time $\tilde O(n^{2/3})$, our algorithm needs more runtime since comparing elements takes time $\Omega(1)$. More precisely, each comparison takes time $O(\sqrt{d})$ in the following way: In order to compare two elements of the two sets, we can use Grover's search to find out if the two substrings are different in any position and if so we can find the leftmost position in time $O(\sqrt{d})$. Thus, it takes time $O(\sqrt{d})$ to compare two elements which results in runtime $\tilde O(n^{2/3} \sqrt{d})$.

\begin{lemma}\label{lemma:firstone}
	One can in time $\tilde O(n^{2/3}\sqrt{d})$ determine if the two strings have a common substring of size $d$ with a quantum algorithm.
\end{lemma}

\paragraph*{Quantum algorithm for large $d$.}
Next, we discuss an algorithm that runs in time $\tilde O(n/\sqrt{d})$ and verifies if there is a common substring of length $d$ between the two strings. %Combining that with Lemma \ref{lemma:firstone} yields an algorithm with runtime $\tilde O(n^{5/6})$. 
In our algorithm, we assume that a substring of length $d$ is shared between the two strings and our goal is to find that substring. If we fail to do so, we conclude that the longest common substring between the two strings is smaller than $d$. Let us fix a common substring of size $d$ in the two strings. We mark the first $\lfloor d/3 \rfloor$ characters of that substring in $A$. In our algorithm, we sample a substring of length $2\lfloor d/3 \rfloor$ of $A$ and a substring of length $d$ of $B$. We call the substring sampled from $A$ the pattern and denote it by $P$ and denote the substring sampled from $B$ by $S$. Also, let the starting positions be $x$ and $y$, respectively. Our aim is to guarantee that the substring sampled from $A$ starts from a marked character and the substring sampled from $B$ contains $P$ and more generally contains the $P$ part of the optimal solution in $B$. That is, if we extend $S$ from both ends by $\lfloor d/3 \rfloor$, it contains the optimal solution.

Let us first compute the probability of sampling such $P$ and $S$. There are at least $\lfloor d/3 \rfloor$ marked characters in $A$ and thus with probability $d/n/3$ we sample the right pattern. Moreover, the corresponding substring of solution in $B$ has at least $\lfloor d/3 \rfloor$ positions such that if we sample $S$ starting from those positions the pair $(P,S)$ is desirable. Thus, with probability $\Omega(d^2/n^2)$ we sample a desired pair $(S,P)$ and therefore via amplitude amplification~\cite{brassard2002quantum} we can guarantee such a choice with probability $2/3$ only by incurring a multiplicative factor $O(n/d)$ to the runtime. From here on, we assume that our choice of $S$ and $P$ meets our expectation.
\input{figs/lcs1}

Next, we aim to find positions of $S$ that match with $P$. For this purpose, we use the string matching algorithm of Ramesh and Vinay~\cite{ramesh2003string} that searches $P$ in $S$ in time $\tilde O(\sqrt{|S|}+\sqrt{|P|})$. If there is no matches, then we can imply that $S$ and $P$ do not meet our property and therefore this should not happen. If there is one such position, then we can detect in time $\sqrt{d}$ if by extending this matching from two ends we can obtain a common substring of size $d$. We use Grover's search to find the left-most (up to $d$ characters away) position where the two substrings differ when extending them from right. We do the same from the left and it tells us if this gives a common substring of size at least $d$. Each search takes time $O(\sqrt{d})$.

More generally, the above idea works when there are only $O(1)$ many positions of $S$ that match with $P$. However, we should address the case that $P$ appears many times in $S$. Indeed, this only happens if $P$ is periodic. In the following, we discuss how this can can be handled. In time $O(\sqrt{d})$ we find the leftmost and rightmost positions of $S$ that match with $P$. Let the starting index of the leftmost match be $\ell$ and the starting index of the rightmost match be $r$. In other words, $P = S[\ell, \ell+|P|-1] = S[r,r+|P|-1]$. Since $|S| = d$ and we have $P = 2\lfloor d/3 \rfloor$ then the two substrings overlap. Therefore, $P$ as well as the entire string $S[\ell, r+|P|-1]$ is $(r-\ell)$-periodic.

\input{figs/f1}
\input{figs/f2}
\input{figs/f3}
Let us denote the substring $B[\ell, r+|P|-1]$ by $T$. We extend both $P$ and $T$ from left and right up to a distance of $2d$ in the following way: We increase the index of the ending point so long as the substring remains $(r-\ell)$-periodic. We also stop if we move the ending point by more than $2d$. We do the same for the starting point; we decrease the starting point so long as the substring remains $(r-\ell)$-periodic and up to at most a distance of $2d$. Since we bound the maximum change by $2d$, then this can be done in time $O(\sqrt{d})$ via Grover's search. Let us denote the resulting substrings by $A[\alpha,\beta]$ and $B[\alpha',\beta']$. The following observation enables us to find the solution in time $O(\sqrt{d})$: one of the following three cases holds for the optimal solution:
\begin{enumerate}
	\item The starting index of the corresponding optimal solution in $A$ is smaller than $\alpha$ and thus the corresponding character of $A[\alpha]$ in $B$ is $B[\alpha']$ (Figure \ref{fig:1}). 
	\item The ending  index of the corresponding optimal solution in $A$ is larger than $\beta$ and thus the corresponding character of $A[\beta']$ in $B$ is $B[\beta']$ (Figure \ref{fig:2}). 
	\item The corresponding optimal solution in $A$ is in the interval $A[\alpha,\beta]$ and thus it is $(r-\ell)$-periodic (Figure \ref{fig:3}).
\end{enumerate}

In all three cases, we can find the optimal solution in time $O(\sqrt{b})$. For the first two cases, we know one correspondence between the two common substrings of length $d$. More precisely, in Case 1 we know that $A[\alpha]$ is part of the solution and this character corresponds to $B[\alpha']$. Thus, it suffices to do a Grover's search from two ends to extend the matching in the two directions. Similarly in Case 2 we know that $A[\beta]$ corresponds to $B[\beta']$ and thus via a Grover's search we find a common substring of length $d$ in the two strings.

Finally, for Case 3 we point out that since the entire solution lies in intervals $A[\alpha,\beta]$ and $B[\alpha', \beta']$ then we have $\beta \geq \alpha + d-1$ and $\beta' \geq \alpha' + d-1$. Notice that both intervals $A[\alpha,\beta]$ and $B[\alpha',\beta']$ are $(r-\ell)$-periodic. Let the starting position of $P$ in $A$ be $x$. For a fixed position $y$ in the interval $[\alpha',\beta']$ that matches with $P$, if we extend this matching from the two ends we obtain a solution of size $\min\{x-\alpha,y-\alpha'\} + \min\{\beta-x+1, \beta'-y+1\}$. This means that extending one of the following matchings between $P$ as $S$ gives us a common subsequence of size $d$.

\begin{itemize}
	\item The rightmost matching in the interval $B[\alpha',\alpha'+|P|+(x-\alpha)]$.
	\item The leftmost matching in the interval $B[\alpha'+(x-\alpha),\beta']$.
\end{itemize}

Each matching can be found in time $O(\sqrt{d})$ and similar to the ideas explained above we can extend each matching to verify if it gives us a common substring of size $d$ in time $O(\sqrt{d})$. Therefore, the overall runtime of the algorithm is $\tilde O(n/\sqrt{d})$.

\begin{lemma}\label{lemma:secondone}
	One can in time $\tilde O(n/\sqrt{d})$ determine if the two strings have a common substring of size $d$ with a quantum algorithm.
\end{lemma}

\paragraph*{Combining the two algorithms.}
Combining Lemmas \ref{lemma:firstone} and \ref{lemma:secondone} gives us a solution in time $\tilde O(n^{5/6})$.
\begin{theorem}\label{theorem:lcs-exact}%[as a corollary of Lemmas \ref{lemma:firstone} and \ref{lemma:secondone}]
	Longest common substring of two strings of size $n$ can be computed with a quantum algorithm in time $\tilde O(n^{5/6})$.
\end{theorem}
\begin{proof}
	We start by a binary search on $d$ (size of the solution). To verify a given $d$, we consider two cases: if $d < n^{1/6}$ we run the first algorithm and otherwise we run the second algorithm. Thus, the overall runtime is bounded by $\tilde O(n^{5/6})$.
\end{proof}

\subsection{Quantum algorithm for approximated \textsf{LCS}}\label{sub:lcs-approximate}
In the following, we show that if an approximate solution suffices then we can improve the runtime down to $\tilde O(n^{3/4})$. Similar to the above discussion, we use two algorithms for small $d$ and large $d$. Our algorithm for large $d$ is the same as the one we use for exact solution. For small $d$ we modify the algorithm of Lemma \ref{lemma:firstone} to improve its runtime down to $\tilde O(n^{2/3}d^{1/3})$. This is explained in Lemma~\ref{lemma:3}.

\begin{lemma}\label{lemma:3}
	Given two strings $A$ and $B$ of size $n$ that share a common substring of length $d$, for any constant $0 < \epsilon < 1$ we can find a common substring of length $(1-\epsilon)d$ between the two strings in time $\tilde O(n^{2/3}d^{1/3})$.
\end{lemma}
\begin{proof}
	Similar to Lemma \ref{lemma:firstone}, we use element distinctness for this algorithm. We make two sets $S_A$ and $S_B$ and prove that they share two equal elements if and only if their corresponding substrings of size $(1-\epsilon)d$ are equal. The difference between this algorithm and the algorithm of Lemma \ref{lemma:firstone} is that here $S_A$ and $S_B$ contain $O(1/\epsilon n/\sqrt{d})$ elements instead of $n-d+1$ elements. Let $k = \epsilon \sqrt{d}$. We break both strings into blocks of size $k$ and make the two sets in the following way:
	\input{figs/f4}
	\begin{itemize}
		\item For each $i$ such that $i \equiv^k 1$, we put element $(A,i)$ in set $S_A$.
		\item For each $i$ such that $\lceil i / k \rceil \equiv^k 1$ we put element $(B,i)$ in set $S_B$.
	\end{itemize}
	It follows that among the $\epsilon d$ first characters of the solution, there is one position which is included in $S_A$ such that its corresponding position in $B$ is also included in $S_B$. Thus, if we define the equality between two element $(A,i)$ and $(B,j)$ as $A[i,i+(1-\epsilon)d-1] = B[j,j+(1-\epsilon)d-1] $ then by solving element distinctness for $S_A$ and $S_B$ we can find a desired solution. Since we have $O(n/\sqrt{d})$ elements in each set then the overall runtime is bounded by $\tilde O((n/\sqrt{d})^{2/3}\sqrt{d}) = \tilde O(n^{2/3}d^{1/3})$.
\end{proof}
Lemmas \ref{lemma:secondone} and \ref{lemma:3} %along with previous algorithms 
lead to a quantum algorithm for \textsf{LCS} with approximation factor $1+\epsilon$ and runtime $\tilde O(n^{3/4})$.
\begin{theorem}\label{theorem:lcs-approx}%[as a corollary of Lemmas \ref{lemma:3} and \ref{lemma:secondone}]
	For any constant $0 < \epsilon < 1$, longest common substring of two strings of size $n$ can be approximated within a factor $1+\epsilon$ with a quantum algorithm in time $\tilde O(n^{3/4})$.
\end{theorem}
\begin{proof}
	We start by a binary search on $d$ (size of the solution). To verify a given $d$, we consider two cases: if $d < n^{1/4}$ we run the first algorithm and otherwise we run the second algorithm. Thus, the overall runtime is bounded by $\tilde O(n^{3/4})$.
\end{proof}

==> src/old files/lcs-perm-old.tex <==
% !TEX root = ../draft.tex
\newcommand{\rr}{r}
\renewcommand{\Cc}{\mathcal{C}}

\section{Longest Common Substring for Permutations}
In this section we consider \textsf{LCS} for permutations, i.e., we assume that $A$ and $B$ are non-repetitive strings. We show that there exist a $\tilde O(n^{3/4})$-time quantum algorithm that computes an exact $\textsf{LCS}$ and a $\tilde O(n^{2/3})$-time quantum algorithm that computes a $(1+\varepsilon)$-approximation of an $\textsf{LCS}$. This significantly improves the results of the previous section. Note that for $(1+\varepsilon)$-approximation our upper bound is tight since the lower bound of Theorem \ref{th:lb-Ulam-approx} also holds for permutations.

%%%%%%%
\subsection{Quantum walks}
We first briefly describe the quantum walk approach to solve element distinctness (and several other problems). 

Let $S$ be a finite set and $r$ be any integer such that $r\le |S|$. Let us write $S_r$ the set of all subsets $R\subseteq S$ of size $r$. Let us fix $S_r^\ast\subseteq S_r$. The elements of $S_r^\ast$ are called the marked sets. 
The quantum walk approach associates to each $R\in S_r$
a database $D(R)$. Three types of cost are associated with~$D$.
The setup cost $s(\rr)$ is the cost to set up the database $D(R)$ for any $R\in S_r$.
The update cost $u(\rr)$ is the cost to update $D(R)$ for any $R\in S_r$: converting $D(R)$ to $D((R\setminus{a})\cup \{a'\})$ for any $a\in R$ and $a'\in S\backslash R$. 
The checking cost $c(\rr)$ is the cost of checking, given $D(R)$ for any $R\in S_r$, if $R\in S_r^\ast$. 
The techniques developed by Ambainis \cite{AmbainisSICOMP07}, which combine Grover search
and quantum walks, can then be used to find with high probability one marked set $R$.
We will use in this paper the following statement (we refer to \cite{AmbainisSICOMP07, Magniez+SICOMP11} for details). 
\begin{proposition}[\cite{AmbainisSICOMP07}]\label{fact_magniez}
Consider any value $\rr\in\{1,\ldots,|S|\}$ and any constant $\gamma>0$.
Assume that either $S_r^\ast=\emptyset$ or $\frac{|S_r^\ast|}{|S_r|}\ge \delta$ holds, for some known value $\delta>0$.
There exists a quantum algorithm that always rejects if $S_r^\ast=\emptyset$, 
outputs a set $R\in S_r^\ast$ with probability at least $1-\frac{1}{n^\gamma}$ otherwise, and has complexity 
\[
\tilde O\left(s(\rr)+\sqrt{1/\delta}\left(\sqrt{\rr}\times u(\rr)+c(\rr)\right)\right).
\]
\end{proposition} 
%\noindent While the upper bound of Proposition% \ref{fact_magniez} will be sufficient for our purpose, 
%let us mention that better upper bounds can be obtained using recent developments on quantum search by quantum walks 
%(see \cite{Magniez+SICOMP11}).  

Let us now explain how to solve element distinctness using this framework. Assume that the input is $x_1,\ldots,x_n$. We set $S=[1\ldots n]$ and say that a set $R\in S_r$ is marked if there exists a pair $(i,j)\in R\times R$ such that $i\neq j$ and $x_i=x_j$. Easy calculations show that the fraction of marked sets is $\Omega(r^2/n^2)$. By using a cleverly designed data structure, which is a combination of a hash table and a skip list (see \cite{AmbainisSICOMP07} for details), we can have $s(r)=\tilde O (r)$ and $u(r)=c(r)=\tilde O(\log n)$. 
From Proposition~\ref{fact_magniez}, the overall complexity of the quantum walk is thus
\[
\tilde O\left(r+\frac{n}{r}\left(\sqrt{\rr}\times 1+1\right)\right).
\]
By taking $r=n^{2/3}$ we get complexity $\tilde O(n^{2/3})$. 


%%%%%
\subsection{Exact algorithm for \textsf{LCS} of permutations}
We set $S=[1,n-d+1]$. Below we assume that $r\ge 2$ (the value of $r$ will be set at the end of the algorithm).
For any set $R\in S_r$ we define the data structure $D(R)$ as follows:
\begin{itemize}
\item
$D(R)$ records all the values $A[k]$ and $B[k]$ for all $k\in R$ using two instances of the data structure considered in the element distinctness algorithm from \cite{AmbainisSICOMP07};
\item
additionally, $D(R)$ records the number of pairs $(i,j)\in R\times R$ such that $A[i]=B[j]$;
\item
additionally, if the number of pairs $(i,j)\in R\times R$ such that $A[i]=B[j]$ is at most $\ceil{100r^2/n}$ then $D(R)$ stores explicitly all these pairs; otherwise $D(R)$ simply stores the first $\ceil{100r^2/n}$ such pairs (here we use the index $i$ to decide the order).
\end{itemize}
We define the set of marked sets $S_r^\ast$ as follows. We say that $R$ is marked if the following two conditions hold:
\begin{itemize}
\item[(i)]
there exists a pair $(i,j)\in R\times R$ such that $A[i\dots i+d-1]=B[j\ldots j+d-1]$;
\item[(ii)]
the number of pairs $(i,j)\in R\times R$ such that $A[i]=B[j]$ is at most $\ceil{100r^2/n}$.
\end{itemize}
The following lemma is easy to show.
\begin{lemma}\label{lemma:ratio}
Assume that $r^2\ge (n\log n)^2$.
If $A$ and $B$ have a common subsequence of length $d$, then the fraction of marked sets is 
$\Omega\left(r^2/n^2\right)$.
\end{lemma}
\begin{proof}
The fraction of sets $R$ for which there exists a pair $(i,j)\in R\times R$ such that $A[i\dots i+d-1]=B[j\ldots j+d-1]$ is at least 
\[
\frac{{n-2\choose r-2}}{{n \choose r}}=\frac{r(r-1)}{n(n-1)}\ge \frac{r^2}{2n^2},
\]
where we used our assumption $r\ge 2$ to derive the last inequality. Thus Condition (i) holds with probability at least $r^2/(2n^2)$.

Let $X$ be the random variable representing the number of pairs $(i,j)\in R_1\times R_2$ such that $A[i]=B[j]$ when $(R_1,R_2)$ is taken uniformly at random. We will show that $X\le \ceil{100 r^2/n}$ with high probability. 

We will show an upper bound on $X$ conditioned on the fact that for each $i\in R_1$ there exists an index $j\in S$ such that $A[i]=B[j]$.

Assume that we have fixed $R_1$ and that for each $i\in R_1$ there exists an index $j\in S$ such that $A[i]=B[j]$. Let $Y$ denote the random variable corresponding to $X$ conditioned on this assumption. Observe that $Y$ is an hypergeometric distribution. Its expected value of $Y$ is $r^2/n$. From Chernoff’s bound, we get 
\begin{align*}
\Pr\left[Y \ge \frac{2r^2}{n}\right]\le \exp\left(-\frac{r^2}{n^2}\right)\le \frac{1}{n^2}.
\end{align*}
Thus the fraction of $(R_1,R_2)$ such that Condition (ii) does not hold is at most $1/n^2$.

The statement of the lemma then follows from the union bound.

%Let $m$ denote the number of pairs $(i,j)\in S\times S$ such that $A[i]=B[j]$. Note that $m\in\{1,\ldots,n\}$. When taking a set $R\in S_r$ uniformly at random, the expected number of pairs $(i,j)\in R\times R$ such that $A[i]=B[j]$ is $mr^2/n^2\le r^2/n$. By Markov’s inequality we obtain:
%\begin{align*}
%\Pr_{R\in S_r}\Big[&\textrm{number of pairs $(i,j)\in R\times R$ such that $A[i]=B[j]$ exceeds} \ceil{100r^2/n}\Big]\\
%&\le \Pr_{R\in S_r}\Big[\textrm{number of pairs $(i,j)\in R\times R$ such that $A[i]=B[j]$ exceeds } 100mr^2/n^2\Big]\\
%&\le \frac{1}{100}.
%\end{align*}
%\Francois{This is not enough: we need Chernoff’s inequality. I am trying to do this below.}
%
%Let $e$ be one of these pairs, let $X_e$ be the random variable that takes value 1 if both indices of $e$ are in $R$. The expectation of $X_e$ is 
%\[
%\E[X_e]= \frac{r^2}{n^2}.
%\]
%The number of good pairs in $R\times R$ is $\sum_e X_e$. While the random variables $X_e$ are not iid, they do satisfy Chernoff’s bounds. \Francois{Is it true?} Thus the probability that $R\times R$ does not contain any good pair is 
%\begin{align*}
%\Pr\left[\sum_{e}X_e = 0\right]\le \Pr\left[\sum_{e}X_e \le \frac{mr^2}{4n^2}\right]\le \exp\left(-\frac{mr^2}{16n^2}\right)\le 1-\frac{mr^2}{32n^2},
%\end{align*}
%where we used the fact that $\exp(-x)\le 1-x/2$ on $x\in[0,1]$. Thus the fraction of $R$ such that $R\times R$ contains a good pair is at least $mr^2/(32n^2)$.
%
%
%From the union bound, we conclude that the fraction of marked sets is $\Omega(r^2/n^2)$.
\end{proof}

Let us now analyze the costs corresponding to this quantum walk. The setup and update costs are
$s(r) = \tilde O(r)$ and 
$u(r)=\tilde O(\log n)$.
The checking operation first check if the number of pairs $(i,j)\in R\times R$ such that $A[i]=B[j]$ is at most $\ceil{100r^2/n}$ and then, if this condition is satisfied, performs a Grover search on all pairs $(i,j)\in R\times R$ such that $A[i]=B[j]$ stored in $D(R)$, in order to check if there exists a pair $(i,j)\in R\times R$ such that $A[i\dots i+d-1]=B[j\ldots j+d-1]$. The cost is
\[
c(r) = \tilde O(1+ \sqrt{\ceil{100r^2/n}}\sqrt{d}).
\]
Using Proposition~\ref{fact_magniez}, we get that the overall complexity of the quantum walk is 
\[
\tilde O\left(r+\frac{n}{r}(\sqrt{r}\times 1 + \sqrt{\ceil{100r^2/n}}\sqrt{d})\right)=\tilde O\left(r+\frac{n}{\sqrt{r}}+\sqrt{nd}\right).
\]
For $d\le n^{1/3}$, this expression is minimized for $r=n^{2/3}$ and gives complexity $\tilde O(n^{2/3})$. For $d\ge n^{1/3}$, the complexity is dominated by the last term $\tilde O(\sqrt{nd})$.

By combining the above algorithm with the $\tilde O(n/\sqrt{d})$-time algorithm of Lemma \ref{lemma:3}, we get overall complexity $\tilde O(n^{3/4})$.

%%%%%
\subsection{$(1+\varepsilon)$-Approximation algorithm for \textsf{LCS} of permutations}
We set again $S=[1,n-d+1]$ and, for any $R\in S_r$, we define the data structure $D(R)$ exactly as above.
This time, we say that $R$ is marked if the following two conditions hold:
\begin{itemize}
\item
there exists a pair $(i,j)\in R\times R$ such that $A[i\ldots i+\ceil{(1-\varepsilon)d}-1]=B[j\ldots j+\ceil{(1-\varepsilon)d}-1]$;
\item
the number of pairs $(i,j)\in R\times R$ such that $A[i]=B[j]$ is at most $\ceil{100r^2/n}$.
\end{itemize}
We can show the following lemma similarly to Lemma \ref{lemma:ratio}.
\begin{lemma}\label{lemma:ratio-approx}
Assume that $rd\le n$.
\Francois{This condition is satisfied when we apply this lemma.}
If $A$ and $B$ have a common subsequence of length $d$, then the fraction of marked sets is
$\Omega\left(\frac{dr^2}{n^2}\right)$.
\end{lemma}
\begin{proof}
%\Francois{I am still working on the proof of this lemma.} 
Let us write $m=d-\ceil{(1-\varepsilon) d}$ and say that a pair $(i,j)\in S\times S$ is good if $A[i\ldots i+\ceil{(1-\varepsilon)d}-1]=B[j\ldots j+\ceil{(1-\varepsilon)d}-1]$. There are at least $m$ good pairs in $S\times S$. 
%The probability that $R_1$ does not contain any element involved in a good pair is
%\begin{align*}
%\frac{{n-m\choose r}}{{n \choose r}}&= \left(1-\frac{mr}{n^2}\right)^{n(1\pm O(m^3/n^3+r^3/n^3+1/n))}\\
%&=1-\Omega\left(\frac{rm}{n}\right),
%\end{align*}
%where we used Lemma 3.4 from \cite{magniez2007quantum}.
%%the fact that $\exp(-x)\le 1-x/2$ on $x\in[0,1]$ to derive the last inequality. 
%Thus with probability at least $\Omega(rm/n)=\Omega(rd/n)$, the set $R_1$ contains at least one element involved in a good pair.
The probability that $R_1$ does not contain any element involved in a good pair is
\begin{align*}
\frac{{n-m\choose r}}{{n \choose r}}&= \frac{(n-m)!r!(n-r)!}{r!(n-m-r)!n!}\\
&=\frac{(n-m)(n-m-1)\cdots (n-m-r+1)}{n(n-1)\cdots(n-r+1)}\\
&\le \left(\frac{n-m}{n}\right)^r=\left(1-\frac{m}{n}\right)^r\le \exp\left(-\frac{rm}{n}\right)\\
&\le 1-\frac{rm}{2n},
\end{align*}
where we used the fact that $\exp(-x)\le 1-x/2$ on $x\in[0,1]$ to derive the last inequality. Thus with probability at least $rm/(2n)$, the set $R_1$ contains at least one element involved in a good pair.


Assuming that $R_1$ contains at least one element involved in a good pair, when choosing $R_2$ at random
%the %probability that $R_1\times R_2$ does not contain any good pair is at most 
%\begin{align*}
%\frac{{n-1\choose r}}{{n \choose r}}&= 1-\frac{r}{n},
%\end{align*}
%and thus 
with probability at least $r/n$ it contains a good pair.
Thus the overall probability that $R_1\times R_2$ contains a good pair is at least $\Omega(dr^2/n^2)$.

%Under this assumption, the probability that $R_2$
%
%\begin{align*}
%\sum_{i=0}^{\min(m,r)}&\Pr[\textrm{$R_1$ contains $i$ elements involved in collision}]\cdot \frac{{n-i\choose r}}{{n \choose r}}\\
%&\le \sum_{i=0}^{\min(m,r)}\Pr[\textrm{$R_1$ contains $i$ elements involved in collision}]\cdot \frac{{n-m\choose r}}{{n \choose r}}
%\end{align*}
%\begin{align*}
%\frac{{n-m\choose r}}{{n \choose r}}&= \frac{(n-m)!r!(n-r)!}{r!(n-m-r)!n!}\\
%&=\frac{(n-m)(n-m-1)\cdots (n-m-r+1)}{n(n-1)\cdots(n-r+1)}\\
%&\le \left(\frac{n-m}{n}\right)^r=\left(1-\frac{m}{n}\right)^r\le \exp\left(-\frac{rm}{n}\right)\\
%&\le 1-\frac{rm}{2n},
%\end{align*}
%where we used the fact that $\exp(-x)\le 1-x/2$ on $x\in[0,1]$ to derive the last inequality. 


%Note that all those pairs do not overlap. We now take a set $R$ uniformly at random in $S_r$. For each good pair $e$, let $X_e$ be the random variable that takes value 1 if both indices of $e$ are in $R$. The expectation of $X_e$ is 
%\[
%\E[X_e]=\frac{{n-2\choose r-2}}{{n \choose r}}\ge \frac{r^2}{2n^2}.
%\]
%The number of good pairs in $R\times R$ is $\sum_e X_e$. While the random variables $X_e$ are not iid, they do satisfy Chernoff’s bounds. \Francois{Need to check that this is true.} Thus the probability that $R\times R$ does not contain any good pair is 
%\begin{align*}
%\Pr\left[\sum_{e}X_e = 0\right]\le \Pr\left[\sum_{e}X_e \le \frac{mr^2}{4n^2}\right]\le \exp\left(-\frac{mr^2}{16n^2}\right)\le 1-\frac{mr^2}{32n^2},
%\end{align*}
%where we used the fact that $\exp(-x)\le 1-x/2$ on $x\in[0,1]$. Thus the fraction of $R$ such that $R\times R$ contains a good pair is at least $mr^2/(32n^2)$.
%
%such that $A[i\ldots i+\ceil{(1-\varepsilon)d}-1]=B[j\ldots j+\ceil{(1-\varepsilon)d}-1]$ is thus $mr^2/n^2$.
%\[
%m\cdot\frac{{n-2\choose r-2}}{{n \choose r}}\ge \frac{mr^2}{2n^2}.
%\]
%While 
%
%The probability that a 
%
%The fraction of sets $R$ that contain at least of of such pairs is thus at least 
%\[
%\Theta(\varepsilon d)\cdot\frac{{n-2\choose r-2}}{{n \choose r}}=\Omega\left(\frac{dr^2}{n^2}\right).
%\]

The remaining of the proof is similar to the proof of Lemma \ref{lemma:ratio}.
\end{proof}

We thus get a quantum walk with running time 
\[
\tilde O\left(r+\frac{n}{r\sqrt{d}}(\sqrt{r}\times 1 + \sqrt{\ceil{100r^2/n}}\sqrt{d})\right)
=\tilde O\left(r+\frac{n}{\sqrt{rd}}+\sqrt{n}\right).
\]
If $d\le \sqrt{n}$ then the expression is minimized for $r=n^{2/3}/d^{1/3}$ and the complexity is $\tilde O(n^{2/3}/d^{1/3})$. If $d\ge \sqrt{n}$ then the complexity is $\tilde O(\sqrt{n})$ (we can simply take $r=n/d$ so that the condition of Lemma \ref{lemma:ratio-approx} is satisfied).

The overall complexity of the algorithm is thus $\tilde O(n^{2/3})$.

==> src/old files/lcs_-_old.tex <==
% !TEX root = ../draft.tex
\section{Longest Common Substring}
In longest common substring, we are given two strings $A$ and $B$ of size $n$ and the goal is to find the largest string $t$ which is a substring of both $A$ and $B$. This problem can be solved in time $O(n)$ via suffix tree in the classic setting. In this section, we give an upper bound and a lower bound for the quantum complexity of this problem. We first begin by giving an exact algorithm for \textsf{LCS} that runs in time $\tilde O(n^{5/6})$. In our algorithm, we do a binary search on the size of the solution. We denote this value by $d$. Thus, by losing an $O(\log n)$ factor in the runtime, we reduce the problem to verifying if a substring of size $d$ is shared between the two strings. Our approach is twofold; we design separate algorithms for small and large $d$.

Our algorithm for small $d$ is inspired by a variant of \textit{element distinctness}. In this variant, two sets of pointers $S_A$ and $S_B$ are given and the goal is to verify if the two sets share a common element. It has been shown~\cite{ambainis2007quantum} that element distinctness can be solved in time $\tilde O(n^{2/3})$ if the number of elements in the two sets is equal to $n$. Moreover, the algorithm uses oracle queries that compare the elements. The total number of queries made to the oracle is also $\tilde O(n^{2/3})$~\cite{ambainis2007quantum}. For small $d$, we use element distinctness. Let $|\Sigma|$ be the size of the alphabet and $v:\Sigma \rightarrow [0,|\Sigma|-1]$ be a function that maps every element of the alphabet to a distinct number in range $0 \ldots |\Sigma|-1$. In other words, $v$ is a perfect hashing for the characters. We extend this definition to substrings of the two strings. For a string $t$, we define $v(t)$ as follows:

$$v(t) = \sum_{i = 1}^{|t|} v(t_i) |\Sigma|^{i-1}.$$

It follows from the definition that two strings $t_1$ and $t_2$ are equal if and only if we have $v(t_1) = v(t_2)$. From the two strings, we make two sets of numbers $S_A$ and $S_B$ each having $n-d+1$ elements. Element $i$ of set $S_A$ is a pair $(A,i)$ whose value is equal to $v(A[i,i+d-1])$ and similarly element $i$ of $S_B$ is a pair $(B,i)$ whose value is equal to $v(B[i,i+d-1])$. Note that the size of the representation for each element is $O(1)$ but comparing elements takes time $\Omega(1)$. The two sets contain elements with equal values if and only if the two strings have a common substring of size $d$. Therefore, by solving element distinctness for $S_A$ and $S_B$ we can find out if the size of the solution is at least $d$. Although element distinctness can be solved in time $\tilde O(n^{2/3})$, our algorithm needs more runtime since comparing elements takes time $\Omega(1)$. More precisely, each comparison takes time $O(\sqrt{d})$ in the following way: In order to compare two elements of the two sets, we can use Grover's search to find out if the two substrings are different in any position and if so we can find the leftmost position in time $O(\sqrt{d})$. Thus, it takes time $O(\sqrt{d})$ to compare two elements which results in runtime $\tilde O(n^{2/3} \sqrt{d})$.

\begin{lemma}\label{lemma:firstone}
	One can in time $\tilde O(n^{2/3}\sqrt{d})$ determine if the two strings have a common substring of size $d$ with a quantum algorithm.
\end{lemma}

Next, we discuss an algorithm that runs in time $\tilde O(n/\sqrt{d})$ and verifies if there is a common substring of length $d$ between the two strings. Combining that with Lemma \ref{lemma:firstone} yields an algorithm with runtime $\tilde O(n^{5/6})$. In our algorithm, we assume that a substring of length $d$ is shared between the two strings and our goal is to find that substring. If we fail to do so, we conclude that the longest common substring between the two strings is smaller than $d$. Let us fix a common substring of size $d$ in the two strings. We mark the first $\lfloor d/3 \rfloor$ characters of that substring in $A$. In our algorithm, we sample a substring of length $2\lfloor d/3 \rfloor$ of $A$ and a substring of length $d$ of $B$. We call the substring sampled from $A$ the pattern and denote it by $P$ and denote the substring sampled from $B$ by $S$. Also, let the starting positions be $x$ and $y$, respectively. Our aim is to guarantee that the substring sampled from $A$ starts from a marked character and the substring sampled from $B$ contains $P$ and more generally contains the $P$ part of the optimal solution in $B$. That is, if we extend $S$ from both ends by $\lfloor d/3 \rfloor$, it contains the optimal solution.

Let us first compute the probability of sampling such $P$ and $S$. There are at least $\lfloor d/3 \rfloor$ marked characters in $A$ and thus with probability $d/n/3$ we sample the right pattern. Moreover, the corresponding substring of solution in $B$ has at least $\lfloor d/3 \rfloor$ positions such that if we sample $S$ starting from those positions the pair $(P,S)$ is desirable. Thus, with probability $\Omega(d^2/n^2)$ we sample a desired pair $(S,P)$ and therefore via amplitude amplification~\cite{brassard2002quantum} we can guarantee such a choice with probability $2/3$ only by incurring a multiplicative factor $O(n/d)$ to the runtime. From here on, we assume that our choice of $S$ and $P$ meets our expectation.
\input{figs/lcs1}

Next, we aim to find positions of $S$ that match with $P$. For this purpose, we use the string matching algorithm of Ramesh and Vinay~\cite{ramesh2003string} that searches $P$ in $S$ in time $\tilde O(\sqrt{|S|}+\sqrt{|P|})$. If there is no matches, then we can imply that $S$ and $P$ do not meet our property and therefore this should not happen. If there is one such position, then we can detect in time $\sqrt{d}$ if by extending this matching from two ends we can obtain a common substring of size $d$. We use Grover's search to find the left-most (up to $d$ characters away) position where the two substrings differ when extending them from right. We do the same from the left and it tells us if this gives a common substring of size at least $d$. Each search takes time $O(\sqrt{d})$.

More generally, the above idea works when there are only $O(1)$ many positions of $S$ that match with $P$. However, we should address the case that $P$ appears many times in $S$. Indeed, this only happens if $P$ is periodic. In the following, we discuss how this can can be handled. In time $O(\sqrt{d})$ we find the leftmost and rightmost positions of $S$ that match with $P$. Let the starting index of the leftmost match be $\ell$ and the starting index of the rightmost match be $r$. In other words, $P = S[\ell, \ell+|P|-1] = S[r,r+|P|-1]$. Since $|S| = d$ and we have $P = 2\lfloor d/3 \rfloor$ then the two substrings overlap. Therefore, $P$ as well as the entire string $S[\ell, r+|P|-1]$ is $(r-\ell)$-periodic.

\input{figs/f1}
\input{figs/f2}
\input{figs/f3}
Let us denote the substring $B[\ell, r+|P|-1]$ by $T$. We extend both $P$ and $T$ from left and right up to a distance of $2d$ in the following way: We increase the index of the ending point so long as the substring remains $(r-\ell)$-periodic. We also stop if we move the ending point by more than $2d$. We do the same for the starting point; we decrease the starting point so long as the substring remains $(r-\ell)$-periodic and up to at most a distance of $2d$. Since we bound the maximum change by $2d$, then this can be done in time $O(\sqrt{d})$ via Grover's search. Let us denote the resulting substrings by $A[\alpha,\beta]$ and $B[\alpha',\beta']$. The following observation enables us to find the solution in time $O(\sqrt{d})$: one of the following three cases holds for the optimal solution:
\begin{enumerate}
	\item The starting index of the corresponding optimal solution in $A$ is smaller than $\alpha$ and thus the corresponding character of $A[\alpha]$ in $B$ is $B[\alpha']$ (Figure \ref{fig:1}). 
	\item The ending  index of the corresponding optimal solution in $A$ is larger than $\beta$ and thus the corresponding character of $A[\beta']$ in $B$ is $B[\beta']$ (Figure \ref{fig:2}). 
	\item The corresponding optimal solution in $A$ is in the interval $A[\alpha,\beta]$ and thus it is $(r-\ell)$-periodic (Figure \ref{fig:3}).
\end{enumerate}

In all three cases, we can find the optimal solution in time $O(\sqrt{b})$. For the first two cases, we know one correspondence between the two common substrings of length $d$. More precisely, in Case 1 we know that $A[\alpha]$ is part of the solution and this character corresponds to $B[\alpha']$. Thus, it suffices to do a Grover's search from two ends to extend the matching in the two directions. Similarly in Case 2 we know that $A[\beta]$ corresponds to $B[\beta']$ and thus via a Grover's search we find a common substring of length $d$ in the two strings.

Finally, for Case 3 we point out that since the entire solution lies in intervals $A[\alpha,\beta]$ and $B[\alpha', \beta']$ then we have $\beta \geq \alpha + d-1$ and $\beta' \geq \alpha' + d-1$. Notice that both intervals $A[\alpha,\beta]$ and $B[\alpha',\beta']$ are $(r-\ell)$-periodic. Let the starting position of $P$ in $A$ be $x$. For a fixed position $y$ in the interval $[\alpha',\beta']$ that matches with $P$, if we extend this matching from the two ends we obtain a solution of size $\min\{x-\alpha,y-\alpha'\} + \min\{\beta-x+1, \beta'-y+1\}$. This means that extending one of the following matchings between $P$ as $S$ gives us a common subsequence of size $d$.

\begin{itemize}
	\item The rightmost matching in the interval $B[\alpha',\alpha'+|P|+(x-\alpha)]$.
	\item The leftmost matching in the interval $B[\alpha'+(x-\alpha),\beta']$.
\end{itemize}

Each matching can be found in time $O(\sqrt{d})$ and similar to the ideas explained above we can extend each matching to verify if it gives us a common substring of size $d$ in time $O(\sqrt{d})$. Therefore, the overall runtime of the algorithm is $\tilde O(n/\sqrt{d})$.

\begin{lemma}\label{lemma:secondone}
	One can in time $\tilde O(n/\sqrt{d})$ determine if the two strings have a common substring of size $d$ with a quantum algorithm.
\end{lemma}

Combining Lemmas \ref{lemma:firstone} and \ref{lemma:secondone} gives us a solution in time $\tilde O(n^{5/6})$.
\begin{theorem}\label{theorem:lcs}[as a corollary of Lemmas \ref{lemma:firstone} and \ref{lemma:secondone}]
	Longest common substring of two strings of size $n$ can be computed with a quantum algorithm in time $\tilde O(n^{5/6})$.
\end{theorem}
\begin{proof}
	We start by a binary search on $d$ (size of the solution). To verify a given $d$, we consider two cases: if $d < n^{1/6}$ we run the first algorithm and otherwise we run the second algorithm. Thus, the overall runtime is bounded by $\tilde O(n^{5/6})$.
\end{proof}

In the following, we show that if an approximate solution suffices then we can improve the runtime down to $\tilde O(n^{3/4})$. Similar to the above discussion, we use two algorithms for small $d$ and large $d$. Our algorithm for large $d$ is the same as the one we use for exact solution. For small $d$ we modify the algorithm of Lemma \ref{lemma:firstone} to improve its runtime down to $\tilde O(n^{2/3}d^{1/3})$. This is explained in Lemma \ref{lemma:3}.

\begin{lemma}\label{lemma:3}
	Given two strings $A$ and $B$ of size $n$ that share a common substring of length $d$, for any constant $0 < \epsilon < 1$ we can find a common substring of length $(1-\epsilon)d$ between the two strings in time $\tilde O(n^{2/3}d^{1/3})$.
\end{lemma}
\begin{proof}
	Similar to Lemma \ref{lemma:firstone}, we use element distinctness for this algorithm. We make two sets $S_A$ and $S_B$ and prove that they share two equal elements if and only if their corresponding substrings of size $(1-\epsilon)d$ are equal. The difference between this algorithm and the algorithm of Lemma \ref{lemma:firstone} is that here $S_A$ and $S_B$ contain $O(1/\epsilon n/\sqrt{d})$ elements instead of $n-d+1$ elements. Let $k = \epsilon \sqrt{d}$. We break both strings into blocks of size $k$ and make the two sets in the following way:
	\input{figs/f4}
	\begin{itemize}
		\item For each $i$ such that $i \equiv^k 1$, we put element $(A,i)$ in set $S_A$.
		\item For each $i$ such that $\lceil i / k \rceil \equiv^k 1$ we put element $(B,i)$ in set $S_B$.
	\end{itemize}
	It follows that among the $\epsilon d$ first characters of the solution, there is one position which is included in $S_A$ such that its corresponding position in $B$ is also included in $S_B$. Thus, if we define the equality between two element $(A,i)$ and $(B,j)$ as $A[i,i+(1-\epsilon)d-1] = B[j,j+(1-\epsilon)d-1] $ then by solving element distinctness for $S_A$ and $S_B$ we can find a desired solution. Since we have $O(n/\sqrt{d})$ elements in each set then the overall runtime is bounded by $\tilde O((n/\sqrt{d})^{2/3}\sqrt{d}) = \tilde O(n^{2/3}d^{1/3})$.
\end{proof}
Lemma \ref{lemma:secondone} along with previous algorithms leads to a quantum algorithm for \textsf{LCS} with approximation factor $1+\epsilon$ and runtime $\tilde O(n^{3/4})$.
\begin{theorem}\label{theorem:lcs}[as a corollary of Lemmas \ref{lemma:3} and \ref{lemma:secondone}]
	For any constant $0 < \epsilon < 1$, longest common substring of two strings of size $n$ can be approximate within a factor $1+\epsilon$ with a quantum algorithm in time $\tilde O(n^{3/4})$.
\end{theorem}
\begin{proof}
	We start by a binary search on $d$ (size of the solution). To verify a given $d$, we consider two cases: if $d < n^{1/4}$ we run the first algorithm and otherwise we run the second algorithm. Thus, the overall runtime is bounded by $\tilde O(n^{3/4})$.
\end{proof}

\Francois{
Here are some ideas about how to improve the running time for special types of inputs. For a string $A$ of length $n$, an integer $t\in[1,n]$, and any integer $i\in[1,n-t]$, let us define $C_{A,t}(i)$ as the maximum, over all the subset $S\subseteq [1,n-t]\setminus\{i\}$ of size $O(\log n)$, of the quantity
\[
\sum_{j\in S}\sqrt{n-H(A[i,i+t-1],A[j,j+t-1])},
\]
where $H$ denote the Hamming distance. This notion can be interpreted as follows: if $C_{A,t}(i)$ is small then the substring $A[i,\ldots,i+t-1]$ is easy to compare to the other substrings of $A$ or length $t$ (since their Hamming distance is large). Now define the quantity
\[
\textsf{cost}(A,t)=\sum_{i=1}^{n-t} C_{A,t}(i).
\]
I believe that we can reduce the complexity of Lemmas 2 and 5 in the case where $\textsf{cost}(A,t)$ and $\textsf{cost}(B,t)$ are small since $\textsf{cost}(A,t)+\textsf{cost}(B,t)$ is precisely the average setup cost of the quantum walks.
More precisely, I think we can show the following.
\begin{proposition}
Assume that $\textsf{cost}(A,t)=\tilde O(n)$ and $\textsf{cost}(B,t)=\tilde O(n)$ for all $t\ge 1$. Then the LCS can be computed exactly in $\tilde O(n^{3/4})$ time and can be approximated within a factor $1+\epsilon$ in $\tilde O(n^{2/3})$ time.
\end{proposition}
Note that the assumption of this proposition are satisfied, for example, if $A$ and $B$ are random strings, or if $A$ and $B$ are non-repetitive strings.
}


==> src/old files/lcs_-_old2.tex <==
% !TEX root = ../draft.tex
\section{Longest Common Substring}
In longest common substring, we are given two strings $A$ and $B$ of size $n$ and the goal is to find the largest string $t$ which is a substring of both $A$ and $B$. This problem can be solved in time $O(n)$ via suffix tree in the classic setting. In this section, we give an upper bound and a lower bound for the quantum complexity of this problem. We first begin by giving an exact algorithm for \textsf{LCS} that runs in time $\tilde O(n^{5/6})$. In our algorithm, we do a binary search on the size of the solution. We denote this value by $d$. Thus, by losing an $O(\log n)$ factor in the runtime, we reduce the problem to verifying if a substring of size $d$ is shared between the two strings. Our approach is twofold; we design separate algorithms for small and large $d$.

\paragraph*{Exact quantum algorithm for small $d$.}
Our algorithm for small $d$ is inspired by a variant of \textit{element distinctness}. In this variant, two sets of pointers $S_A$ and $S_B$ are given and the goal is to verify if the two sets share a common element. It has been shown~\cite{ambainis2007quantum} that element distinctness can be solved in time $\tilde O(n^{2/3})$ if the number of elements in the two sets is equal to $n$. Moreover, the algorithm uses oracle queries that compare the elements. The total number of queries made to the oracle is also $\tilde O(n^{2/3})$~\cite{ambainis2007quantum}. For small $d$, we use element distinctness. Let $|\Sigma|$ be the size of the alphabet and $v:\Sigma \rightarrow [0,|\Sigma|-1]$ be a function that maps every element of the alphabet to a distinct number in range $0 \ldots |\Sigma|-1$. In other words, $v$ is a perfect hashing for the characters. We extend this definition to substrings of the two strings. For a string $t$, we define $v(t)$ as follows:

$$v(t) = \sum_{i = 1}^{|t|} v(t_i) |\Sigma|^{i-1}.$$

It follows from the definition that two strings $t_1$ and $t_2$ are equal if and only if we have $v(t_1) = v(t_2)$. From the two strings, we make two sets of numbers $S_A$ and $S_B$ each having $n-d+1$ elements. Element $i$ of set $S_A$ is a pair $(A,i)$ whose value is equal to $v(A[i,i+d-1])$ and similarly element $i$ of $S_B$ is a pair $(B,i)$ whose value is equal to $v(B[i,i+d-1])$. Note that the size of the representation for each element is $O(1)$ but comparing elements takes time $\Omega(1)$. The two sets contain elements with equal values if and only if the two strings have a common substring of size $d$. Therefore, by solving element distinctness for $S_A$ and $S_B$ we can find out if the size of the solution is at least $d$. Although element distinctness can be solved in time $\tilde O(n^{2/3})$, our algorithm needs more runtime since comparing elements takes time $\Omega(1)$. More precisely, each comparison takes time $O(\sqrt{d})$ in the following way: In order to compare two elements of the two sets, we can use Grover's search to find out if the two substrings are different in any position and if so we can find the leftmost position in time $O(\sqrt{d})$. Thus, it takes time $O(\sqrt{d})$ to compare two elements which results in runtime $\tilde O(n^{2/3} \sqrt{d})$.

\begin{lemma}\label{lemma:firstone}
	One can in time $\tilde O(n^{2/3}\sqrt{d})$ determine if the two strings have a common substring of size $d$ with a quantum algorithm.
\end{lemma}

\paragraph*{Exact quantum algorithm for large $d$.}
Next, we discuss an algorithm that runs in time $\tilde O(n/\sqrt{d})$ and verifies if there is a common substring of length $d$ between the two strings. Combining that with Lemma \ref{lemma:firstone} yields an algorithm with runtime $\tilde O(n^{5/6})$. In our algorithm, we assume that a substring of length $d$ is shared between the two strings and our goal is to find that substring. If we fail to do so, we conclude that the longest common substring between the two strings is smaller than $d$. Let us fix a common substring of size $d$ in the two strings. We mark the first $\lfloor d/3 \rfloor$ characters of that substring in $A$. In our algorithm, we sample a substring of length $2\lfloor d/3 \rfloor$ of $A$ and a substring of length $d$ of $B$. We call the substring sampled from $A$ the pattern and denote it by $P$ and denote the substring sampled from $B$ by $S$. Also, let the starting positions be $x$ and $y$, respectively. Our aim is to guarantee that the substring sampled from $A$ starts from a marked character and the substring sampled from $B$ contains $P$ and more generally contains the $P$ part of the optimal solution in $B$. That is, if we extend $S$ from both ends by $\lfloor d/3 \rfloor$, it contains the optimal solution.

Let us first compute the probability of sampling such $P$ and $S$. There are at least $\lfloor d/3 \rfloor$ marked characters in $A$ and thus with probability $d/n/3$ we sample the right pattern. Moreover, the corresponding substring of solution in $B$ has at least $\lfloor d/3 \rfloor$ positions such that if we sample $S$ starting from those positions the pair $(P,S)$ is desirable. Thus, with probability $\Omega(d^2/n^2)$ we sample a desired pair $(S,P)$ and therefore via amplitude amplification~\cite{brassard2002quantum} we can guarantee such a choice with probability $2/3$ only by incurring a multiplicative factor $O(n/d)$ to the runtime. From here on, we assume that our choice of $S$ and $P$ meets our expectation.
\input{figs/lcs1}

Next, we aim to find positions of $S$ that match with $P$. For this purpose, we use the string matching algorithm of Ramesh and Vinay~\cite{ramesh2003string} that searches $P$ in $S$ in time $\tilde O(\sqrt{|S|}+\sqrt{|P|})$. If there is no matches, then we can imply that $S$ and $P$ do not meet our property and therefore this should not happen. If there is one such position, then we can detect in time $\sqrt{d}$ if by extending this matching from two ends we can obtain a common substring of size $d$. We use Grover's search to find the left-most (up to $d$ characters away) position where the two substrings differ when extending them from right. We do the same from the left and it tells us if this gives a common substring of size at least $d$. Each search takes time $O(\sqrt{d})$.

More generally, the above idea works when there are only $O(1)$ many positions of $S$ that match with $P$. However, we should address the case that $P$ appears many times in $S$. Indeed, this only happens if $P$ is periodic. In the following, we discuss how this can can be handled. In time $O(\sqrt{d})$ we find the leftmost and rightmost positions of $S$ that match with $P$. Let the starting index of the leftmost match be $\ell$ and the starting index of the rightmost match be $r$. In other words, $P = S[\ell, \ell+|P|-1] = S[r,r+|P|-1]$. Since $|S| = d$ and we have $P = 2\lfloor d/3 \rfloor$ then the two substrings overlap. Therefore, $P$ as well as the entire string $S[\ell, r+|P|-1]$ is $(r-\ell)$-periodic.

\input{figs/f1}
\input{figs/f2}
\input{figs/f3}
Let us denote the substring $B[\ell, r+|P|-1]$ by $T$. We extend both $P$ and $T$ from left and right up to a distance of $2d$ in the following way: We increase the index of the ending point so long as the substring remains $(r-\ell)$-periodic. We also stop if we move the ending point by more than $2d$. We do the same for the starting point; we decrease the starting point so long as the substring remains $(r-\ell)$-periodic and up to at most a distance of $2d$. Since we bound the maximum change by $2d$, then this can be done in time $O(\sqrt{d})$ via Grover's search. Let us denote the resulting substrings by $A[\alpha,\beta]$ and $B[\alpha',\beta']$. The following observation enables us to find the solution in time $O(\sqrt{d})$: one of the following three cases holds for the optimal solution:
\begin{enumerate}
	\item The starting index of the corresponding optimal solution in $A$ is smaller than $\alpha$ and thus the corresponding character of $A[\alpha]$ in $B$ is $B[\alpha']$ (Figure \ref{fig:1}). 
	\item The ending  index of the corresponding optimal solution in $A$ is larger than $\beta$ and thus the corresponding character of $A[\beta']$ in $B$ is $B[\beta']$ (Figure \ref{fig:2}). 
	\item The corresponding optimal solution in $A$ is in the interval $A[\alpha,\beta]$ and thus it is $(r-\ell)$-periodic (Figure \ref{fig:3}).
\end{enumerate}

In all three cases, we can find the optimal solution in time $O(\sqrt{b})$. For the first two cases, we know one correspondence between the two common substrings of length $d$. More precisely, in Case 1 we know that $A[\alpha]$ is part of the solution and this character corresponds to $B[\alpha']$. Thus, it suffices to do a Grover's search from two ends to extend the matching in the two directions. Similarly in Case 2 we know that $A[\beta]$ corresponds to $B[\beta']$ and thus via a Grover's search we find a common substring of length $d$ in the two strings.

Finally, for Case 3 we point out that since the entire solution lies in intervals $A[\alpha,\beta]$ and $B[\alpha', \beta']$ then we have $\beta \geq \alpha + d-1$ and $\beta' \geq \alpha' + d-1$. Notice that both intervals $A[\alpha,\beta]$ and $B[\alpha',\beta']$ are $(r-\ell)$-periodic. Let the starting position of $P$ in $A$ be $x$. For a fixed position $y$ in the interval $[\alpha',\beta']$ that matches with $P$, if we extend this matching from the two ends we obtain a solution of size $\min\{x-\alpha,y-\alpha'\} + \min\{\beta-x+1, \beta'-y+1\}$. This means that extending one of the following matchings between $P$ as $S$ gives us a common subsequence of size $d$.

\begin{itemize}
	\item The rightmost matching in the interval $B[\alpha',\alpha'+|P|+(x-\alpha)]$.
	\item The leftmost matching in the interval $B[\alpha'+(x-\alpha),\beta']$.
\end{itemize}

Each matching can be found in time $O(\sqrt{d})$ and similar to the ideas explained above we can extend each matching to verify if it gives us a common substring of size $d$ in time $O(\sqrt{d})$. Therefore, the overall runtime of the algorithm is $\tilde O(n/\sqrt{d})$.

\begin{lemma}\label{lemma:secondone}
	One can in time $\tilde O(n/\sqrt{d})$ determine if the two strings have a common substring of size $d$ with a quantum algorithm.
\end{lemma}

\paragraph*{Combining the two algorithms.}
Combining Lemmas \ref{lemma:firstone} and \ref{lemma:secondone} gives us a solution in time $\tilde O(n^{5/6})$.
\begin{theorem}\label{theorem:lcs-exact}%[as a corollary of Lemmas \ref{lemma:firstone} and \ref{lemma:secondone}]
	Longest common substring of two strings of size $n$ can be computed with a quantum algorithm in time $\tilde O(n^{5/6})$.
\end{theorem}
\begin{proof}
	We start by a binary search on $d$ (size of the solution). To verify a given $d$, we consider two cases: if $d < n^{1/6}$ we run the first algorithm and otherwise we run the second algorithm. Thus, the overall runtime is bounded by $\tilde O(n^{5/6})$.
\end{proof}

\paragraph*{Approximate solution.}
In the following, we show that if an approximate solution suffices then we can improve the runtime down to $\tilde O(n^{3/4})$. Similar to the above discussion, we use two algorithms for small $d$ and large $d$. Our algorithm for large $d$ is the same as the one we use for exact solution. For small $d$ we modify the algorithm of Lemma \ref{lemma:firstone} to improve its runtime down to $\tilde O(n^{2/3}d^{1/3})$. This is explained in Lemma \ref{lemma:3}.

\begin{lemma}\label{lemma:3}
	Given two strings $A$ and $B$ of size $n$ that share a common substring of length $d$, for any constant $0 < \epsilon < 1$ we can find a common substring of length $(1-\epsilon)d$ between the two strings in time $\tilde O(n^{2/3}d^{1/3})$.
\end{lemma}
\begin{proof}
	Similar to Lemma \ref{lemma:firstone}, we use element distinctness for this algorithm. We make two sets $S_A$ and $S_B$ and prove that they share two equal elements if and only if their corresponding substrings of size $(1-\epsilon)d$ are equal. The difference between this algorithm and the algorithm of Lemma \ref{lemma:firstone} is that here $S_A$ and $S_B$ contain $O(1/\epsilon n/\sqrt{d})$ elements instead of $n-d+1$ elements. Let $k = \epsilon \sqrt{d}$. We break both strings into blocks of size $k$ and make the two sets in the following way:
	\input{figs/f4}
	\begin{itemize}
		\item For each $i$ such that $i \equiv^k 1$, we put element $(A,i)$ in set $S_A$.
		\item For each $i$ such that $\lceil i / k \rceil \equiv^k 1$ we put element $(B,i)$ in set $S_B$.
	\end{itemize}
	It follows that among the $\epsilon d$ first characters of the solution, there is one position which is included in $S_A$ such that its corresponding position in $B$ is also included in $S_B$. Thus, if we define the equality between two element $(A,i)$ and $(B,j)$ as $A[i,i+(1-\epsilon)d-1] = B[j,j+(1-\epsilon)d-1] $ then by solving element distinctness for $S_A$ and $S_B$ we can find a desired solution. Since we have $O(n/\sqrt{d})$ elements in each set then the overall runtime is bounded by $\tilde O((n/\sqrt{d})^{2/3}\sqrt{d}) = \tilde O(n^{2/3}d^{1/3})$.
\end{proof}
Lemmas \ref{lemma:secondone} and \ref{lemma:3} %along with previous algorithms 
lead to a quantum algorithm for \textsf{LCS} with approximation factor $1+\epsilon$ and runtime $\tilde O(n^{3/4})$.
\begin{theorem}\label{theorem:lcs-approx}%[as a corollary of Lemmas \ref{lemma:3} and \ref{lemma:secondone}]
	For any constant $0 < \epsilon < 1$, longest common substring of two strings of size $n$ can be approximated within a factor $1+\epsilon$ with a quantum algorithm in time $\tilde O(n^{3/4})$.
\end{theorem}
\begin{proof}
	We start by a binary search on $d$ (size of the solution). To verify a given $d$, we consider two cases: if $d < n^{1/4}$ we run the first algorithm and otherwise we run the second algorithm. Thus, the overall runtime is bounded by $\tilde O(n^{3/4})$.
\end{proof}

==> src/old files/lps-old.tex <==
% !TEX root = ../draft.tex
\section{Longest Palindrome Substring}\label{section:lps}
Longest palindrome substring (\textsf{LPS}) is a famous problem in computer science. \textsf{LPS} can be solved in linear time via suffix tree. In this section, we present a quantum algorithm that solves \textsf{LPS} in time $\tilde O(\sqrt{n})$. We complement this result by a lower bound of $\tilde \Omega(\sqrt{n})$ for quantum algorithms even for the special case of 0/1 strings.

Our algorithm starts with a binary search on the size of the solution. We use $l$ and $u$ as a lower bound and an upper bound on the size of the solution. Initially we set $l = 1$ and $u = n$. Each time we set $d = \lceil (l+u)/2 \rceil$ and try to find a solution of size at least $d$. If such a solution exists, then we continue on by setting $l = d$. Otherwise we set $u = d-1$. After $O(\log n)$ steps we have $l = u$ which is equal to the size of the solution. Thus, in the following, we assume that an integer $d$ is given and our goal is to find out if a solution of size at least $d$ exists in the string.

One thing to keep in mind is that if the solution size is larger than $d$, we may not necessarily have a palindrome substring of size $d$ but in that case, we certainly have a palindrome substring of size $d+1$. Thus, all it takes to verify if the solution size is at least $d$ is to look for a solution of size either $d$ or $d+1$. We consider each case separately. Thus, from here on, we assume that our string contains a palindrome substring of size $d$ and we wish to find such a substring.

When $d$ is a constant, we can find the solution via Grover's search in time $O(\sqrt{n})$. Thus, without loss of generality we assume that $d > 10$.  Before explaining the algorithm, we bring some definitions which give more intuition about the algorithm. Let interval $[\ell, \ell+d-1]$ be a palindrome substring of length $d$. We mark the first $\lfloor d/2 \rfloor$ characters of this interval. Since we may have several palindrome substrings of length $d$ we may have more than $d/2$ marked characters in our string. However, since there is at least one solution of size $d$, then the number of marked characters is at least $\Omega(d)$. In our algorithm, each time we sample one character of the string in the hope that it is a marked character. Thus, each time with probability at least $\Omega(d/n)$ we sample a marked character. By quantum amplitude amplification~\cite{brassard2002quantum}, with an overhead of  $O(\sqrt{n/d})$ in the runtime, one can guarantee that a marked character is sampled once with probability at least $2/3$ in one of the runs.

Let position $r$ be a marked character that our algorithm samples. We define a string $S$ of length $d$ that spans the interval $[r,r+d-1]$ of the input string. We also define  a pattern $P$ of length $\lceil d/2 \rceil$ which is equal to the reverse of interval $[r, r+\lceil d/2 \rceil -1]$. \Francois{It may be a good idea to put the paragraph discussing the intuition of the algorithm here, before introducing Lemma 6.} We say a position $i$ of $S$ matches with pattern $P$ if $S[i,i+|P|-1] = P$. In our algorithm, we find all positions of the $S$ that match with pattern $P$. We show in the following that this can be done in time $\tilde O(\sqrt{d})$.

\begin{lemma}\label{lemma:per}
	For strings $S$ and $P$ constructed as explained above, there is a quantum algorithm that lists all occurrences of $P$ in $S$ in time $\tilde O(\sqrt{d})$. The algorithm is randomized and succeeds with high probability.
\end{lemma}
\begin{proof}
To do so, we first find the rightmost occurrence of the $P$ in $S$ using the quantum algorithm of Ramesh and Vinay~\cite{ramesh2003string}. This takes time $\tilde O(\sqrt{d})$ since $|S|+|P| = O(d)$. If $P$ does not appear in $S$ at all or only once, we are done. Otherwise, let $o_r$ be the rightmost position of $S$ that matches with $P$. That is $S[o_r,o_r+|P|-1] = P$. Moreover, let $o$ be the position of  the second rightmost occurrence of $P$ in $S$. We argue that $T = \{ o_r - i(o_r - o) | 0 \leq i \leq \lfloor (o_r-1) / (o_r-o) \rfloor \}$ is the set of all occurrences of $P$ in $S$. More precisely, every element of $T$ is the starting position of an occurance of $P$ in $S$. Since $|S| \leq 2|P|$, there is one special case in which $o = o_r - |P|$ in which case $|T|$ contains exactly two elements and the proof is trivial. Thus, we assume in the following that the two rightmost occurrences of $P$ in $S$ overlap. 

We say a string $s$ is $q$-periodic if we have $s_i = s_{i+q}$ for all $1 \leq i \leq |s|-q$. Since $P$ appears as a substring of $S$ at both at locations $o_r$ and $o$ then $P$ is $(o_r-o)$-periodic. Moreover, $P$ is not $i$-periodic for any $1 < i < o_r - o$ since otherwise $o$ would not be the position of the second rightmost occurrence of $P$ in $S$. We first prove that each element of $T$ is a position in $S$ that matches with $P$. Recall that by the way we construct $S$ and $P$, $P$ is equal to the reverse of the first $|P|$ characters of $S$. Moreover, $|S| \leq 2|P|$ and thus the entire interval $S[1,o_r+|P|-1]$ is $(o_r-o)$-periodic.\Francois{I don’t understand the last step of the argument: why does this show that the entire interval is $(o_r-o)$-periodic?} This implies that every element of $T$ is the beginning of one occurrence of $P$ in $S$.

\input{figs/periodic.tex}

In order to show that $T$ contains all occurrences of $P$ in $S$, assume for the sake of contradiction that there is a position $p$ of $S$ that is the beginning of one occurrence of $P$ but $p$ is not included in $T$. This implies that there is one element $e \in T$ such that $|e-p| < o_r - o$. Thus, with the same argument $P$ is $|e-p|$-periodic. This is in contradiction with what we proved previously. 
\end{proof}

Before explaining the rest of the algorithm, we bring one observation that gives intuition about the algorithm. We assume that position $r$ of the input string is a marked point. Let $\ell$ be the left most character of such a solution. That is, substring $[\ell, \ell+d-1]$ of the input array is palindrome. Moreover, position $r$ is one of first $\lfloor d/2 \rfloor$ characters of this interval. Since $A[\ell, \ell+d-1]$ is palindrome then we have $A[r+\lceil d/2 \rceil]$ is equal to the reverse of $A[2\ell+d-\lceil d/2 \rceil-r , 2\ell+d-r-1]$.

\input{figs/pattern.tex}

$r$ is marked and therefore it is in the left half of the palindrome substring. Moreover, the size of $S$ is equal to $d$ and by the way we construct $P$ it is equal to the reverse of $A[r+\lceil d/2 \rceil]$. Thus, $A[2\ell+d-\lceil d/2 \rceil-r , 2\ell+d-r-1]$ is equal to $P$ and completely lies inside $S$. Thus, by finding all location of $S$ that match with $P$, we definitely find $A[2\ell+d-\lceil d/2 \rceil-r , 2\ell+d-r-1]$. Define the center of a palindrome substring as the average of its starting position and its ending position (it is not integer if the length of the palindrome substring is even). If we fix a center $c$, one can via Grover's search determine  in time $O(\sqrt{d})$ whether size of the corresponding palindrome substring is at least $d$ or not. 

Recall from the proof of Lemma~\ref{lemma:per} that $T$ is the set of the starting positions of each occurrence of $P$ in $S$. In our algorithm we define a set $C = \{ (r+e + \lceil d/2 \rceil -2)/2  | e \in T\}$ as the set of all possible centers for the solution.  Since we consider all occurrences of $P$ in $S$, by the above argument, one of the elements in $C$ is equal to the actual center of our solution. If $|C| = O(1)$, one can iterate over all elements of $C$ and verify in time $O(\sqrt{d})$ if each one is a center for a palindrome substring of size $d$. Thus, we only need to worry about the runtime if $|C|$ is large. In the following, we show that even if $|C|$ is large, we can narrow down the search to a constant number of elements in $C$ which makes it possible to find a palindrome substring of length $d$.

We show in Lemma \ref{lemma:per} that $C$ is large only if $P$ is periodic. Let $\alpha$ be the periodicity of $P$. As we discuss in Lemma \ref{lemma:per}, every consecutive pair of elements in $T$ have distance $\alpha$. \Francois{Perhaps we can mention these properties directly in the statement of Lemma 6 (or in a new lemma)  --- I think this would be easier to read than referring to the proof of a lemma.} Thus, each pair of consecutive elements in $C$ have distance $\alpha/2$. Let $y$ be the largest index of $A$ such that $A[r,y]$ is $\alpha$-periodic. Also, let $x$ be the smallest index of $A$ such that $A[x,y]$ is periodic. We prove two things in the following: 1) if $y-x \geq d+\alpha$ then we already have a palindrome substring of size $d$ in the interval $[x,y]$ that can easily found in time $O(\sqrt{d})$. 2) Otherwise the center of our solution has a distance of at most $\alpha/2$ from $(x+y)/2$, and thus we only need to consider a constant number of elements in $C$, which enables us to solve the problem in time $O(\sqrt{d})$ as well.

\begin{lemma}
	If $y-x+1 \geq d+\alpha-1$ then one can find a palindrome substring of size at least $d$ in time $O(\sqrt{d})$.
\end{lemma}
\begin{proof}
	
		\input{figs/palindrome}
	Let $e \in T$ be an arbitrary element of $T$. This means that $P = A[r+e-1,r+e-1+|P|-1]$. Since $A[r,r+|P|-1]$ is equal to the reverse of $P$ and the two intervals $[r,r+|P|-1]$ and $[r+e-1,r+e-1+|P|-1]$ overlap then $A[r+e-1,r+e-1+|P|-1]$ is a palindrome substring. Recall that $P$ is $\alpha$-periodic and thus so is the entire substring $A[r,r+e-1+|P|-1]$. This implies that interval $[r,r+e-1+|P|-1]$ is inside interval $[x,y]$. We start by $x' = r$ and $y' = r+e-1+|P|-1$. Next, we shift $[x',y']$ by multiples of $\alpha$ until $||x-x'|-|y-y'|| < \alpha$. Since $A[x,y]$ is $\alpha$-periodic, we still have $A[x',y'] = A[r,r+e-1+|P|-1]$ and therefore $A[x',y']$ is palindrome. Finally, we set $x'' = x' - \min\{|x-x'|,|y-y'|\}$ and $y'' = y'+ \min\{|x-x'|,|y-y'|\}$. It follows from the periodicity of $A[x,y]$ that $A[x'',y'']$ is palindrome. Moreover, the size of $[x'',y'']$ is at most $\alpha-1$ smaller that the size of $[x,y]$. Thus, $A[x'',y'']$ is a desired substring.
	

	
	It is easy to find such a solution in time $O(\sqrt{d})$. The only part of the proof which is non-trivial from a computational standpoint is finding $[x,y]$. If $y-x = O(d)$ then one can find it via Grover's search in time $O\sqrt{d})$. Otherwise, instead of finding $x$ and $y$, we extend $r$ from both ends up to a distance of $2d$ so long as it remains $\alpha$-periodic. This can be done in time $O(\sqrt{d})$ and then with the same analysis we can find a palindrome substring of size at least $d$.
\end{proof}

Finally, we show that if
$y-x+1 \leq d+\alpha$
 then we only need to consider a constant number of candidates for the center of the solution.

\begin{lemma}\label{lemma:2}
   If $y-x+1 < d+\alpha-1$ then the center of the solution cannot be more than $2\alpha$ away from $(x+y)/2$.
\end{lemma}
\begin{proof}
	\input{figs/example}
   We denote the optimal solution by $A[\ell, \ell+d-1]$. Let $c = \ell + (d-1)/2$ be the center of the solution. Assume for the sake of contradiction that $c < (x+y)/2-2\alpha$. This means that $\ell < x-\alpha$. Thus, the interval $A[x-\alpha,x-1]$ is exactly equal to the interval $A[x,x+\alpha-1]$ and thus $A[x-\alpha,y]$ is also $\alpha$-periodic. This is in contradiction wit the maximality of $[x,y]$. A similar proof holds for the case that $c > (x+y)/2+2\alpha$.
\end{proof}

Lemma \ref{lemma:2} implies that we only need to consider all candidates in $C$ that are within the range $[(x+y)/2-2\alpha,(x+y)/2+2\alpha]$. Moreover, the distance between every pair of candidates in $C$ is $\alpha/2$ and therefore we only need to consider a constant number of elements. Therefore, we can find the solution in time $O(\sqrt{d})$. This in addition to the additional multiplicative factor $O(\sqrt{n/d})$ for amplitude amplification gives us a solution in time $\tilde O(\sqrt{n})$. We thus obtain the following result.
\begin{theorem}\label{theorem:lps}
	Longest palindrome substring of a string of size $n$ can be computed with a quantum algorithm in time $\tilde O(\sqrt{n})$.
\end{theorem}


==> src/old files/ulam-distance-eps-old.tex <==
% !TEX root = ../draft.tex
\providecommand{\proc}{\mathrm{XLI_2}}

%========================================================
\section{$(1+\varepsilon)$-Approximation of the Ulam distance}
%========================================================
In this section we prove the following theorem.
\begin{theorem}
For any $\varepsilon>0$, there is a quantum algorithm that computes a $(1+\epsilon)$-approximation of the Ulam distance of two non-repetitive strings in time $\tilde O(\sqrt{n})$.
\end{theorem}

%=========================================
\subsection{Overview of the Classical Algorithm}
%=========================================
In this subsection we describe the relevant results from \cite{Naumovitz+SODA17}.

We first introduce the notion of indicator.
\begin{definition}[\cite{Naumovitz+SODA17}]
Let $P$ be a nonnegative parameter which has an upper bound $r$. A $(\beta_0,\beta_1)$-quality $P$-indicator is a 0-1 value random variable $Z_P$ such that 
\[
\Pr[Z_P=1]\in\left[\frac{P}{r}-\beta_0,\frac{P}{r}+\beta_0\right].
\] 
\end{definition}

We now introduce the notion of gap test.
\begin{definition}
A $(\tau,\delta)$-gap test for $P$ takes as inputs two parameters $a$ and $b$ such that $b>(1+\tau)a$ and outputs SMALL or BIG. The gap test is said to fail if either $P\le a-\delta$ and it outputs BIG, or $P>b$ and it outputs SMALL. 
\end{definition}

The following proposition shows how to convert a gap test with $\delta=0$ into an approximation algorithm.
\begin{proposition}[Proposition 2.1 in \cite{Naumovitz+SODA17}]
A $(\tau,0)$-gap test for $P$ can be converted into a $(1+2\tau+\tau^2)$-approximation algorithm for $P$ with only a logarithmic overhead in the complexity.
\end{proposition}
The following proposition shows that even if $\delta\neq 0$, we can still convert a gap test into an approximation algorithm if $\beta_0$ and $\beta_1$ are approximate multiples of the parameter $P$.
\begin{proposition}[Proposition 3.2 in \cite{Naumovitz+SODA17}]
Let $G$ be a $(\tau,\eta(P+1))$-gap test for $P$. Then $G$ is a $(\tau+2\eta,0)$-gap test for $P$ for input thresholds $a, b$ with $a\ge 1$. 
\end{proposition}

The following proposition shows how to convert an indicator into a gap test.
\begin{proposition}[Proposition 3.1 in \cite{Naumovitz+SODA17}]
Let $\Aa$ be a $(\beta_0,\beta_1)$-quality $P$-indicator. For any $\tau>0$, we can construct a $(\tau,(\beta_0+\beta_1)r)$-gap test for $P$ that works for any thresholds $a\ge (\beta_0+\beta_1)r$ and $b>(1+\tau)a$, and runs in time $O(\frac{(1+\tau)r}{b\tau^3})$ times the running time of $\Aa$.
\end{proposition}

Finally, let us state one of the main algorithmic results of \cite{Naumovitz+SODA17}.
\begin{proposition}
There exists a procedure, named $\proc$, that runs in time $\tilde O(\sqrt{n})$
%\[
%\tilde O\left(\sqrt{\frac{b\edit}{n}}+1\right)
%\]
and is a $(\beta_0,\beta_1)$-quality $Xloss$-indicator
\end{proposition}

\subsection{The quantum algorithm}
%=====================================
%=====================================



==> src/old files/ulam-distance-eps-old_2.tex <==
% !TEX root = ../draft.tex
\providecommand{\proc}{\mathrm{XLI_2}}

%========================================================
\section{$(1+\varepsilon)$-Approximation of the Ulam distance}
%========================================================
In this section we prove the following theorem.
\begin{theorem}\label{th:Ulam-eps}
For any $\varepsilon>0$, there is a quantum algorithm that computes a $(1+\varepsilon)$-approximation of the Ulam distance of two non-repetitive strings in time $\tilde O(\sqrt{n})$.
\end{theorem}

%===========================================
\subsection{Preliminaries}
%=========================================
\paragraph*{Constructing indicators for the Ulam distance.}
%=========================================
We first describe the result from \cite{Naumovitz+SODA17} on which our quantum algorithm will be based.

We first introduce the notion of indicator.
\begin{definition}[\cite{Naumovitz+SODA17}]
Let $P$ be a nonnegative parameter which has an upper bound $r$. A $(\beta_0,\beta_1)$-quality $P$-indicator is a 0-1 value random variable $Z_P$ such that 
\[
\Pr[Z_P=1]\in\left[\frac{P}{r}-\beta_0,\frac{P}{r}+\beta_1\right].
\] 
\end{definition}

%We now introduce the notion of gap test.
%\begin{definition}
%A $(\tau,\delta)$-gap test for $P$ takes as inputs two parameters $a$ and $b$ such that $b>(1+\tau)a$ and outputs SMALL or BIG. The gap test is said to fail if either $P\le a-\delta$ and it outputs BIG, or $P>b$ and it outputs SMALL. 
%\end{definition}
%
%The following proposition shows how to convert a gap test with $\delta=0$ into an approximation algorithm.
%\begin{proposition}[Proposition 2.1 in \cite{Naumovitz+SODA17}]
%A $(\tau,0)$-gap test for $P$ can be converted into a $(1+2\tau+\tau^2)$-approximation algorithm for $P$ with only a logarithmic overhead in the complexity.
%\end{proposition}
%The following proposition shows that even if $\delta\neq 0$, we can still convert a gap test into an approximation algorithm if $\beta_0$ and $\beta_1$ are approximate multiples of the parameter $P$.
%\begin{proposition}[Proposition 3.2 in \cite{Naumovitz+SODA17}]
%Let $G$ be a $(\tau,\eta(P+1))$-gap test for $P$. Then $G$ is a $(\tau+2\eta,0)$-gap test for $P$ for input thresholds $a, b$ with $a\ge 1$. 
%\end{proposition}
%
%The following proposition shows how to convert an indicator into a gap test.
%\begin{proposition}[Proposition 3.1 in \cite{Naumovitz+SODA17}]
%Let $\Aa$ be a $(\beta_0,\beta_1)$-quality $P$-indicator. For any $\tau>0$, we can construct a $(\tau,(\beta_0+\beta_1)r)$-gap test for $P$ that works for any thresholds $a\ge (\beta_0+\beta_1)r$ and $b>(1+\tau)a$, and runs in time $O(\frac{(1+\tau)r}{b\tau^3})$ times the running time of $\Aa$.
%\end{proposition}

Ref.~\cite{Naumovitz+SODA17} showed how to construct an indicator for the Ulam distance:
\begin{proposition}\label{prop:Ulam}
Let $\delta$ be any constant.
Let $A$ and $B$ be two non-repetitive strings of length $n$. For any $t\ge\edit(A,B)$, their exists a $\tilde O(\sqrt{t})$-time classical algorithm that is a $(\beta_0,\beta_1)$-quality $\edit(A,B)$-indicator with upper bound $r=n+t$ and
\[
\beta_0=\delta\cdot \frac{\edit(A,B)}{r} \:\:\:\textrm{ and }\:\:\: \beta_1=\delta \cdot\frac{\edit(A,B)+1}{r}.
\]
\end{proposition}

%%===============================================
%\paragraph*{Approximation algorithms from gap tests.}
%%===============================================
%We now introduce the notion of gap test.
%\begin{definition}
%A $\tau$-gap test for $\edit(A,B)$ takes as inputs two parameters $a$ and $b$ such that $b>(1+\tau)a$ and outputs SMALL or BIG. The gap test is said to fail if either $\edit(A,B)\le a$ and it outputs BIG, or $\edit(A,B)>b$ and it outputs SMALL. 
%\end{definition}
%
%The following proposition shows how to efficiently convert a gap test into an approximation algorithm.
%\begin{proposition}[Proposition 2.1 in \cite{Naumovitz+SODA17}]\label{prop:conv}
%A $\tau$-gap test for $\edit(A,B)$ can be converted into a $(1+2\tau+\tau^2)$-approximation algorithm for $\edit(A,B)$ with only a logarithmic overhead in the complexity.
%\end{proposition}

%===============================================
\paragraph*{Quantum amplitude estimation.}
%===============================================
Our quantum algorithm relies on quantum amplitude amplification. Here is the precise statement of this method.

\begin{theorem}[Theorem 12 in \cite{brassard2002quantum}]\label{th:ae}
Let $\Aa$ be a classical algorithm that runs in time $T$, outputs~$1$ with probability $p$ and outputs $0$ with probability $1-p$, for some (unknown) value $p\in [0,1]$. For any integer $t\ge 1$, there exists a quantum algorithm what runs in time $\tilde O(tT)$ and outputs with high probability an estimate $\tilde p$ such that
\[
|p-\tilde p|\le 2\pi\frac{\sqrt{p(1-p)}}{t}+\frac{\pi^2}{t^2}.
\]
\end{theorem}
We will actually use the following corollary.
\begin{corollary}\label{cor:ae}
Let $\Aa$ be a classical algorithm that runs in time $T$, outputs~$1$ with probability $p$ and outputs $0$ with probability $1-p$, for some (unknown) value $p\in [q,1/2]$, where $q>0$ is a known lower bound.
For any $\alpha>0$, there exists a quantum algorithm what runs in time $\tilde O(\frac{1}{\alpha\sqrt{q}}T)$ and outputs with high probability an estimate $\tilde p$ such that
\[
(1-\alpha)p\le \tilde p\le (1+\alpha) p.
\]
\end{corollary}
\begin{proof}
Apply Theorem \ref{th:ae} with $t=\Theta\left(\frac{1}{\alpha\sqrt{q}}\right)$.
\end{proof}
%===================================
\subsection{The quantum algorithm}
%===================================
Theorem \ref{th:Ulam-eps} is shown by applying quantum amplitude estimation on the algorithm from Proposition~\ref{prop:Ulam} in order to construct a $\tilde O(\sqrt{n})$-time quantum algorithm $\Qq$ that gives a $(1+\varepsilon)$-approximation of $\edit(A,B)$. 

We now give a sketch of the construction. Here we assume for simplicity that we already know a constant-factor approximation $D(A,B)$ of the quantity $\edit(A,B)$ --- it should be possible to remove this assumption with further work (or we can simply use the algorithm of Section 5 to get a constant-factor approximation).

When choosing $\delta=\Theta(\varepsilon)$ appropriately and $t=D(A,B)$, the classical algorithm of Proposition~\ref{prop:Ulam} (which we refer to as Algorithm $\Aa$) runs in time $\tilde O(\sqrt{\edit(A,B)})$ and outputs $1$ with probability $p$ such that
\[
|p-\edit(A,B)/n|\le c p
\] 
for some $c=\Theta(\varepsilon)$.
 Algorithm $\Qq$ applies quantum amplitude estimation (Corollary \ref{cor:ae}) on $\Aa$ with $\alpha=\Theta(\varepsilon)$ and $q=\Theta(D(A,B)/n)$ to obtain an estimator $\tilde p$ of the probability $p$, and then outputs $n\tilde p$. This gives a $(1+\varepsilon)$-approximation of $\edit(A,B)$. The running time of $\Qq$ is 
 \[
 \tilde O(\sqrt{n/D(A,B)}\times \sqrt{\edit(A,B)})=\tilde O(\sqrt{n}).
 \]


%that performs a $\Theta(\varepsilon)$-gap test for $\edit(A,B)$. This gap test can then be (classically) converted into a $(1+\varepsilon)$-approximation algorithm for $\edit(A,B)$ using Proposition \ref{prop:conv}, with only a logarithmic overhead in the complexity.

%We now describe the quantum algorithm $\Qq$. Let $(a,b)$ be the two input parameters of the gap test. The classical algorithm of Proposition \ref{prop:conv} (which we refer to as Algorithm $\Aa$) outputs a $(1+\Theta(\varepsilon))$-approximation of the quantity $\edit(A,B)/n$ when choose $\delta=\Theta(\varepsilon)$ appropriately.

%Algorithm $\Qq$ applies quantum amplitude estimation on the algorithm from Proposition \ref{prop:Ulam} with $m=\Theta(a/\delta^2)$ with precision parameter $\alpha=??$.

%=====================================
%=====================================



==> src/old files/ulam-distance-eps_-_Copy.tex <==
% !TEX root = ../draft.tex
\providecommand{\proc}{\mathrm{XLI_2}}
\providecommand{\Xloss}{\mathrm{Xloss}}
\providecommand{\Est}[1]{\textsf{QTest}(#1)}
\providecommand{\myLARGE}{\textsf{LARGE}}
\providecommand{\mySMALL}{\textsf{SMALL}}
\providecommand{\Error}{\textsf{ERROR}}
%========================================================
\section{$(1+\epsilon)$-Approximation of the Ulam distance}\label{sec:Ulam}
\color{blue}
Comments from the reviewers:
\begin{itemize}
	\item In Section 6.2 the authors make a mention of UlamEst (twice) without ever defining it in the entire paper.
	
	\item In the same Section 6.2 they say they set the parameter k=... in Theorem 7, but there is no mention of the parameter k in Theorem 7.
	
	\item  The statement of Theorem 7 mentions “...outputs with high probability...”. They use Theorem 7 to prove the claim of Proposition 3 where they without explaining translate **high probability** to $8/\pi^2$. I don’t understand how they get that. However, this is not a major concern as $8/\pi^2$ is indeed a high probability.
	
	\item I don’t understand how they arrive at the last inequality on Page 27. It appears as if with the chosen value of $r$, the inequality holds.
	
	\item  In the proof of Theorem 6, I don’t understand how they get the last term on the left-hand side of the complexity analysis of the algorithm that approximately solves Ulam Distance.
	
	\item In the proof of Theorem 10, it is said that there can not be a palindrome of more than three consecutive blocks, can the authors give me some more intuition here?
	
	\item \color{red}The **mistake** in the Ulam Distance section is as follows: Consider the second last paragraph in the proof of Theorem 6, the paragraph that begins with the sentence: “Assume now that $i*\geq 2\ldots$  The first equation at the end of this paragraph seems to have used the inequality in the wrong direction. Fixing that works. However, I don’t see how the authors derive the equation in the third line after having fixed the inequality direction in the equation in line 1 and then line 2.
	
\end{itemize}
\color{black}
%========================================================
In this section we prove the following theorem.
\begin{theorem-repeat}{theorem:ulam}
\TheoremUlam
%For any constant $\epsilon>0$, there is a quantum algorithm that computes a $(1+\epsilon)$-approximation of the Ulam distance of two non-repetitive strings in time $\tilde O(\sqrt{n})$.
\end{theorem-repeat}

%===========================================
\subsection{Classical indicator for the Ulam distance}
%==================
%\paragraph*{Constructing estimators for the Ulam distance.}
%==================
Naumovitz, Saks and Seshadhri \cite{Naumovitz+SODA17} showed how to construct, for any constant $\epsilon>0$,  a classical algorithm that computes a $(1+\epsilon)$-approximation of the Ulam distance of two non-repetitive strings $A,B$ of length~$n$ in time $\tilde O(n/\edit(A,B)+\sqrt{\edit(A,B)})$. Their algorithm is complex: it consists of nine procedures that form a hierarchy of gap tests and estimators, each with successively better run time. The core technique, which lies at the lowest layer of the hierarchy and gives a very good --- but slow --- estimation of the Ulam distance, is a variant of the Saks-Seshadhri algorithm for estimating the longest increasing sequence from~\cite{Saks+FOCS10}. 

For our purpose, we will only need the following result from~\cite{Naumovitz+SODA17}.\footnote{The precise statement of this result appears in Lemma 8.5 and Table 1 in~\cite{Naumovitz+SODA17}. The procedure is denoted $\textsf{XLI}_2$ in~\cite{Naumovitz+SODA17}. Note that the original statement is actually more general: it considers strings $A,B$ of different lengths and gives an indicator for a slightly different quantity (called $\Xloss(A,B)$ in \cite{Naumovitz+SODA17}). When $A$ and $B$ have the same length we have $\Xloss(A,B)=\frac{1}{2}\edit(A,B)$, which gives the statement of Proposition \ref{prop:Ulam}.} %Also note that the condition $t\ge\edit(A,B)$ is not mentioned explicitly, but is implicitly used in the proof of Lemma~8.5 \cite{SS-pers}.}
\begin{proposition}[\cite{Naumovitz+SODA17}]\label{prop:Ulam}
Let $\delta>0$ be any constant. For any two non-repetitive strings $A,B$ of length~$n$ and any integer parameter $t\ge c\cdot\edit(A,B)$ for some constant $c$ depending only on $\delta$, their exists a $\tilde O(\sqrt{t})$-time classical algorithm $\Estimator{A,B,\delta,t}$ that outputs $1$ with some probability $p$ and $0$ with probability $(1-p)$, for some probability $p$ such that 
\[
p\in \left[(1-\delta)\cdot \frac{\edit(A,B)}{n+t},(1+\delta)\cdot \frac{\edit(A,B)}{n+t}+\frac{\delta}{n+t}\right].
\]
\end{proposition}
The procedure of Proposition \ref{prop:Ulam} lies at one of the lowest layers of the hierarchy in \cite{Naumovitz+SODA17}, and works by applying the Saks-Seshadhri algorithm from~\cite{Saks+FOCS10} on randomly chosen substrings of $A$ and~$B$ (of size roughly $t$).\footnote{We stress that this procedure is still too slow to get a $\tilde O(n/\edit(A,B)+\sqrt{\edit(A,B)})$-time classical algorithm. Indeed, getting a good approximation of $\edit(A,B)$ based only on this procedure would require repeating it $\Omega((n+t)/\edit(A,B))$ times, which would require $\Omega(\sqrt{\edit(A,B)}\cdot (n+t)/\edit(A,B))=\Omega(n/\sqrt{\edit(A,B)})$ time. This is why several additional techniques (which lead to several additional layers in the hierarchy) are used in~\cite{Naumovitz+SODA17}.} 
%This provides a good approximation of the edit distance at a cost smaller than for the test performed at the lowest level.

%We will actually use the following application of amplitude amplification.
%\begin{corollary}\label{cor:ae}
%Let $\Aa$ be a classical algorithm that runs in time $T$, outputs~$1$ with probability $p$ and outputs $0$ with probability $1-p$, for some (unknown) value $p\in [q,1/2]$, where $q>0$ is a known lower bound.
%For any $\alpha>0$, there exists a quantum algorithm what runs in time $\tilde O(\frac{1}{\alpha\sqrt{q}}T)$ and outputs with high probability an estimate $\tilde p$ such that
%\[
%(1-\alpha)p\le \tilde p\le (1+\alpha) p.
%\]
%\end{corollary}
%\begin{proof}
%Apply Theorem \ref{th:ae} with $t=\Theta\left(\frac{1}{\alpha\sqrt{q}}\right)$.
%\end{proof}



%===================================
\subsection{Quantum algorithm for the Ulam distance}
%===================================
To prove Theorem \ref{theorem:ulam}, the basic idea is to apply quantum amplitude estimation on the classical algorithm \textsf{UlamEst} from Proposition~\ref{prop:Ulam}. Let us explain this strategy more precisely and show the technical difficulties we need to overcome. Assume that we know that $\edit(A,B)$ is in the interval $[D_1,D_2]$ for some values $D_1$ and $D_2$. We can then use  $\Estimator{A,B,\delta,t}$ with $t=D_2$, and apply the quantum amplitude estimation algorithm of Theorem~\ref{th:ae} to estimate the probability it outputs~1. If we use~$k=\Theta(\sqrt{(n+t)/D_1})=\Theta(\sqrt{n/D_1})$  in Theorem~\ref{th:ae} and $\delta$ small enough, we will get a good approximation of the quantity $\edit(A,B)/(n+t)$, and thus a good approximation of $\edit(A,B)$. The complexity of this strategy is 
$
\tilde O(\sqrt{n/D_1}\cdot \sqrt{D_2}),
$
which is $\tilde O(\sqrt{n})$  when $D_1\approx D_2$. 

The main issue is that we do not know such tight upper and lower bounds on $\edit(A,B)$. Concerning the upper bound, we overcome this difficultly by simply successively trying $D_2=n$, $D_2=(1-\eta) n$, $D_2=(1-\eta)^2 n$, $\ldots$ for some small constant $\eta$. For the lower bound, on the other hand, we cannot simply start with $D_1=1$ and iteratively increase this value, since the cost would be too high: in order to achieve an overall running time of $\tilde O(\sqrt{n})$ we need to keep $D_1\approx D_2$. Instead of estimating the probability that \textsf{UlamEst} outputs 1 using Theorem \ref{th:ae}, which is too costly, we thus design a gap test that enables us to check if this probability is larger than $D_2$ or smaller than $(1-\eta)D_2$ much more efficiently, in time $\tilde O(\sqrt{n/D_2})$. 

We now present the details of our quantum algorithm. Let us first present the gap test.
This test relies on quantum amplitude amplification. Here is the precise statement of quantum amplitude amplification that we will use.

\begin{theorem}[Theorem 12 in \cite{brassard2002quantum}]\label{th:ae}
Let $\Aa$ be a classical algorithm that runs in time $T$, outputs~$1$ with probability $p$ and outputs $0$ with probability $1-p$, for some (unknown) value $p\in [0,1]$. For any integer $t\ge 1$, there exists a quantum algorithm what runs in time $\tilde O(tT)$ and outputs with high probability an estimate $\tilde p$ such that
\[
|p-\tilde p|\le 2\pi\frac{\sqrt{p(1-p)}}{t}+\frac{\pi^2}{t^2}.
\]
\end{theorem}
\Saeed{Reviewer comment: Theorem 7. The rest of this section uses k instead of t for this theorem.}

The gap test is described in the following proposition.
\begin{proposition}\label{prop:qtest}
Let $\Aa$ be a classical algorithm that runs in time $T$, outputs~$1$ with probability $p$ and outputs $0$ with probability $1-p$, for some (unknown) value $p$.
For any $q\in(0,1]$ and any constant $\eta\in(0,1]$, there exists a quantum algorithm denoted $\Est{\Aa,q,\eta}$ what runs in time $\tilde O(T/\sqrt{q})$ and with probability at least $1-\poly(n)$ outputs \myLARGE{} if $p\ge q$ and \mySMALL{} if $p\le(1-\eta)q$.
\end{proposition}
\begin{proof}
Figure \ref{fig:qtest} describes our main quantum gap test. The complexity of this test is $\tilde O(T/\sqrt{q})$, from Theorem \ref{th:ae}. We show below that its success probability is at least $8/\pi^2$. The success probability can then be increased to $1-1/\poly(n)$ by repeating the test $\Theta(\log n)$ times and using majority voting.
\begin{figure}[h!]
\begin{center}
\fbox{
\begin{minipage}{14.5 cm} 
\begin{itemize}
\item[1.]
Apply the algorithm of Theorem \ref{th:ae} with 
$
k=\frac{20}{\eta\sqrt{q}}.
$
Let $\tilde p$ denote the output.
\item[2.]
Output \myLARGE{} if $\tilde p\ge (1-\eta/2)q$ and output \mySMALL{} if $\tilde p<(1-\eta/2)q$.
\end{itemize}
\end{minipage}
}
\end{center}
\vspace{-4mm}
\caption{Quantum gap test.}\label{fig:qtest}
\end{figure}

Let us analyze the success probability of the quantum gap test of Figure \ref{fig:qtest}. Note that Theorem~\ref{th:ae} guarantees that with probability at least $8/\pi^2$ the value $\tilde p$ satisfies the following two inequalities:
\begin{align}\label{ineq1}
\tilde p&\le p+2\pi\eta\frac{\sqrt{p(1-p)}\sqrt{q}}{20} + \pi^2\eta^2 \frac{q}{400},
\end{align}
\begin{align}\label{ineq2}
\tilde p&\ge p-2\pi\eta\frac{\sqrt{p(1-p)}\sqrt{q}}{20} - \pi^2\eta^2 \frac{q}{400}.
\end{align}

Let us first consider the case $p\le (1-\eta)q$. In that case Inequality (\ref{ineq1}) implies
\[
\tilde p \le (1-\eta)q+2\pi\eta \frac{q}{20}+\pi^2\eta^2\frac{q}{400}< (1-\eta/2)q
\]
since $2\pi/20+\pi^2/400<1/2$.
The probability that the algorithm outputs \myLARGE{} is thus at most $1-8/\pi^2$.

Now consider the case $p\ge q$. In that case Inequality (\ref{ineq2}) implies
\begin{align*}
\tilde p&\ge p-2\pi\eta\frac{\sqrt{p}\sqrt{q}}{20} - \pi^2\eta^2 \frac{q}{400}\\
&= \sqrt{p}\left(\sqrt{p}-2\pi\eta\frac{\sqrt{q}}{20}\right)- \pi^2\eta^2 \frac{q}{400}\\
&\ge q -2\pi \eta\frac{q}{20}-\pi^2\eta^2\frac{q}{400}> (1-\eta/2)q.
\end{align*}
The probability that the algorithm outputs \mySMALL{} is thus at most $1-8/\pi^2$.
\end{proof}


%on the algorithm from Proposition~\ref{prop:Ulam}
%If a good estimate $D$ of $\edit(A,B)$ were known, 
%Using Theorem \ref{th:ae}, this would require applying Algorithm $\Estimator{}$ about $\sqrt{n/\edit(A,B)}$ times.

% in order to construct a $\tilde O(\sqrt{n})$-time quantum algorithm that gives a $(1+\epsilon)$-approximation of $\edit(A,B)$.
%\Francois{It would be nice to add a more detailed informal description of the algorithm.}

We are now ready to give the proof of Theorem \ref{theorem:ulam}.
\begin{proof}[Proof of Theorem \ref{theorem:ulam}]
If $\edit(A,B)\ge \sqrt{n}$ then $\edit(A,B)$ can already be computed in $\tilde O(\sqrt{n})$ time by the classical algorithm from \cite{Naumovitz+SODA17}. We thus assume below that $\edit(A,B)\le \sqrt{n}$. We also assume that $\edit(A,B)>0$, since otherwise the two strings are identical, which can be checked in $\tilde O(\sqrt{n})$ time using Grover search.

Below we will invoke Algorithm $\Estimator{A,B,\epsilon/3,t}$ with values of $t$ such that $t\le \sqrt{n}$. Let us call $p_t$ the probability that it outputs $1$. Note that Proposition \ref{prop:Ulam} guarantees that
\begin{equation}\label{rel}
p_t\in \left[(1-\delta)\left(1-\frac{1}{\sqrt{n}}\right)\cdot \frac{\edit(A,B)}{n},(1+\delta)\cdot \frac{\edit(A,B)}{n}+\frac{\delta}{n}\right]
\end{equation}
for any $t\le \sqrt{n}$.

Our quantum algorithm is described in Figure \ref{fig:qalg}.

%Let us fix $\eta=\Theta(\epsilon)$.  We describe the quantum algorithm below.
\begin{figure}[h!]
\begin{center}
\fbox{
\begin{minipage}{13 cm} 
\begin{itemize}
\item[1.]
Set $\eta=\epsilon/10$ and $\delta=\epsilon/3$ and $r=\ceil{\frac{\log((1+\delta)(\sqrt{n}-1)/n)}{\log (1-\eta)}}$. \Saeed{Comment from reviewers: Figure 13, 1. In the definition of $r$, I believe $(1+\delta)$ should be $(1-\delta)$.}
\item[2.] 
For i from $1$ to $r$ do:
\begin{itemize}
\item[2.1.]
Set $q=(1-\eta)^i /\sqrt{n}$ and $t=(1-\eta)^i \sqrt{n}$.
\item[2.2.]
Apply Algorithm $\Est{\Aa,q,\eta}$ with $\Aa=\Estimator{A,B,\delta,t}$. \Saeed{Comment from the reviewers: Figure 13, 2.2. The guarantee of proposition 2 holds under the assumption that $t>c\cdot ud(A,b)$. Using the exact values of $t$ given, this may not be the case depending on $c$, though a constant factor on $t$ when calling UlamIndic should solve this issue.}
\item[2.3.]
If the output is \myLARGE{}, then stop and return $t$.
\end{itemize}
\item[3.]
Return \Error{}.
\end{itemize}
\end{minipage}
}
\end{center}
\vspace{-2mm}
\caption{Quantum algorithm computing a $(1+\epsilon)$-approximation of the Ulam distance of two strings $A$ and $B$.}\label{fig:qalg}
\end{figure}

First observe that the inequality 
\[
(1-\delta)\left(1-\frac{1}{\sqrt{n}}\right)\cdot \frac{\edit(A,B)}{n}\ge (1-\eta)^r/\sqrt{n}
\]
holds, since we are assuming that $\edit(A,B)\ge 1$.
From Proposition \ref{prop:qtest} combined with (\ref{rel}), this means that with probability at least $1-1/\poly(n)$, the algorithm will never reach Step $3$ (and thus does not output \Error{}). In the remaining of the proof, we assume that the algorithm stops before reaching Step 3. Let~$i^\ast$ denote the value of $i$ during the last iteration of the loop of Step 2, and write $q^\ast=(1-\eta)^{i^\ast}/\sqrt{n}$ and $t^\ast=(1-\eta)^{i^\ast}\sqrt{n}$. Observe that the output of the algorithm is $t^\ast$. 

Assume first that $i^\ast=1$. The output is thus $t^\ast=(1-\eta)\sqrt{n}$. Observe that Algorithm $\textsf{QTest}$ then necessarily outputted $\myLARGE$ for $i=1$. Proposition \ref{prop:qtest} guarantees that with probability at least $1-1/\poly(n)$ the inequality $p_{t^\ast}\ge (1-\eta)q^\ast$ holds (otherwise it would have outputted $\mySMALL$). 
This inequality combined with (\ref{rel}) implies that
\[
(1+\delta)\cdot \frac{\edit(A,B)}{n}+\frac{\delta}{n}\ge (1-\eta)q^\ast
\]
and thus the output $t^\ast=nq^\ast$ of the algorithm satisfies the following inequalities:
\begin{align}\label{ineq:UB}
\begin{aligned}
t^\ast&\le ((1+\delta)\cdot \edit(A,B)+\delta)/(1-\eta)\\
&\le (1+2\delta)\cdot\edit(A,B)/ (1-\eta)\\
&\le (1+2\delta)(1+2\eta) \edit(A,B)\\
&\le (1+\epsilon) \edit(A,B),
\end{aligned}
\end{align}
where we used the inequality $1/(1-x)\le 1+2x$, which holds for any $x\in[0,1/2]$. Also note that the inequality 
\[
t^\ast\ge (1-\epsilon)\edit(A,B)
\]
is trivially satisfied since we are assuming $\edit(A,B)\le \sqrt{n}$ and $\eta<\epsilon$.
The output is thus a $(1+\epsilon)$-approximation of $\edit(A,B)$.

Assume now that $i^\ast\ge 2$. 
%\Francois{We also need to consider $i^\ast=1$, but this ``degenerate’’ case is actually easier since we can use the trivial upper bound $\edit(A,B)\le \sqrt{n}$.} 
Observe that Algorithm $\textsf{QTest}$ then necessarily outputted $\myLARGE$ for $i=i^\ast$ and $\mySMALL$ for $i= i^\ast-1$. 
Since it outputted $\myLARGE$ for $i=i^\ast$, Inequalities (\ref{ineq:UB}) hold with probability at least $1-1/\poly(n)$, from exactly the same argument as above. Since the output was $\mySMALL$ for $i=i^\ast-1$, Proposition \ref{prop:qtest} guarantees that with probability at least $1-1/\poly(n)$ the inequality
$
p_{t^\ast/(1-\eta)}\le q^\ast/(1-\eta)
$
holds (otherwise it would have outputted $\myLARGE$).
%\Francois{Maybe add some explanations about why the output of $\textsf{QTest}$ for $i=i^\ast-1$ cannot be directly used (this is because the output of \textsf{QTest} may be wrong near the threshold, so we need a gap to make a correct decision).}
Since $t^\ast=nq^\ast$, this inequality combined with \ref{rel}) implies:
\begin{align*}
t^\ast&\le n(1-\eta)p_{t^\ast/(1-\eta)}\\
&\le (1-\eta)(1-\delta)\left(1-\frac{2}{\sqrt{n}}\right)\cdot \edit(A,B)\\
&\le (1-\epsilon)\cdot \edit(A,B).
\end{align*}
%where we used the inequality $1/(1-x)\le 1+2x$, which holds for any $x\in[0,1/2]$, to derive the last line.
%\Francois{May need to adjust a bit the values of $\eta$ and $\delta$.}

\Saeed{Comment from the reviewers: second to last equation. First, this should be a lower bound on t. Second I think $\frac{2}{\sqrt{n}}$ should be $\frac{1}{\sqrt{n}}$.}

The output of the algorithm is thus a $(1+\epsilon)$-approximation of $\edit(A,B)$ as well. 

The complexity of the algorithm is 
\[
\tilde O\left(\sum_{i=1}^{r} \frac{1}{\sqrt{(1-\eta)^i/\sqrt{n}}}\sqrt{(1-\eta)^i\sqrt{n}}\right)
=
\tilde O\left(\sqrt{n}\right),
\]
as claimed.
\end{proof}

==> src/old files/ulam-distance-eps_-_Copy__2_.tex <==
% !TEX root = ../draft.tex
\providecommand{\proc}{\mathrm{XLI_2}}
\providecommand{\Xloss}{\mathrm{Xloss}}
\providecommand{\Est}[1]{\textsf{QTest}(#1)}
\providecommand{\myLARGE}{\textsf{LARGE}}
\providecommand{\mySMALL}{\textsf{SMALL}}
\providecommand{\Error}{\textsf{ERROR}}
%========================================================
\section{$(1+\epsilon)$-Approximation of the Ulam distance}\label{sec:Ulam}
%========================================================
In this section we prove the following theorem.
\begin{theorem-repeat}{theorem:ulam}
\TheoremUlam
%For any constant $\epsilon>0$, there is a quantum algorithm that computes a $(1+\epsilon)$-approximation of the Ulam distance of two non-repetitive strings in time $\tilde O(\sqrt{n})$.
\end{theorem-repeat}

%===========================================
\subsection{Classical indicator for the Ulam distance}
%==================
%\paragraph*{Constructing estimators for the Ulam distance.}
%==================
Naumovitz, Saks and Seshadhri \cite{Naumovitz+SODA17} showed how to construct, for any constant $\epsilon>0$,  a classical algorithm that computes a $(1+\epsilon)$-approximation of the Ulam distance of two non-repetitive strings $A,B$ of length~$n$ in time $\tilde O(n/\edit(A,B)+\sqrt{\edit(A,B)})$. Their algorithm is complex: it consists of nine procedures that form a hierarchy of gap tests and estimators, each with successively better run time. The core technique, which lies at the lowest layer of the hierarchy and gives a very good --- but slow --- estimation of the Ulam distance, is a variant of the Saks-Seshadhri algorithm for estimating the longest increasing sequence from~\cite{Saks+FOCS10}. 

For our purpose, we will only need the following result from~\cite{Naumovitz+SODA17}.\footnote{The precise statement of this result appears in Lemma 8.5 and Table 1 in~\cite{Naumovitz+SODA17}. The procedure is denoted $\textsf{XLI}_2$ in~\cite{Naumovitz+SODA17}. Note that the original statement is actually more general: it considers strings $A,B$ of different lengths and gives an indicator for a slightly different quantity (called $\Xloss(A,B)$ in \cite{Naumovitz+SODA17}). When $A$ and $B$ have the same length we have $\Xloss(A,B)=\frac{1}{2}\edit(A,B)$, which gives the statement of Proposition \ref{prop:Ulam}.} %Also note that the condition $t\ge\edit(A,B)$ is not mentioned explicitly, but is implicitly used in the proof of Lemma~8.5 \cite{SS-pers}.}
\begin{proposition}[\cite{Naumovitz+SODA17}]\label{prop:Ulam}
Let $\delta>0$ be any constant. For any two non-repetitive strings $A,B$ of length~$n$ and any integer parameter $t\ge c\cdot\edit(A,B)$ for some constant $c$ depending only on $\delta$, there exists a $\tilde O(\sqrt{t})$-time classical algorithm $\Estimator{A,B,\delta,t}$ that outputs $1$ with some probability $p$ and $0$ with probability $(1-p)$, for some probability $p$ such that 
\[
p\in \left[(1-\delta)\cdot \frac{\edit(A,B)}{n+t},(1+\delta)\cdot \frac{\edit(A,B)}{n+t}+\frac{\delta}{n+t}\right].
\]
\end{proposition}
The procedure of Proposition \ref{prop:Ulam} lies at one of the lowest layers of the hierarchy in \cite{Naumovitz+SODA17}, and works by applying the Saks-Seshadhri algorithm from~\cite{Saks+FOCS10} on randomly chosen substrings of $A$ and~$B$ (of size roughly $t$).\footnote{We stress that this procedure is still too slow to get a $\tilde O(n/\edit(A,B)+\sqrt{\edit(A,B)})$-time classical algorithm. Indeed, getting a good approximation of $\edit(A,B)$ based only on this procedure would require repeating it $\Omega((n+t)/\edit(A,B))$ times, which would require $\Omega(\sqrt{\edit(A,B)}\cdot (n+t)/\edit(A,B))=\Omega(n/\sqrt{\edit(A,B)})$ time. This is why several additional techniques (which lead to several additional layers in the hierarchy) are used in~\cite{Naumovitz+SODA17}.} 
%This provides a good approximation of the edit distance at a cost smaller than for the test performed at the lowest level.

%We will actually use the following application of amplitude amplification.
%\begin{corollary}\label{cor:ae}
%Let $\Aa$ be a classical algorithm that runs in time $T$, outputs~$1$ with probability $p$ and outputs $0$ with probability $1-p$, for some (unknown) value $p\in [q,1/2]$, where $q>0$ is a known lower bound.
%For any $\alpha>0$, there exists a quantum algorithm what runs in time $\tilde O(\frac{1}{\alpha\sqrt{q}}T)$ and outputs with high probability an estimate $\tilde p$ such that
%\[
%(1-\alpha)p\le \tilde p\le (1+\alpha) p.
%\]
%\end{corollary}
%\begin{proof}
%Apply Theorem \ref{th:ae} with $t=\Theta\left(\frac{1}{\alpha\sqrt{q}}\right)$.
%\end{proof}



%===================================
\subsection{Quantum algorithm for the Ulam distance}
%===================================
To prove Theorem \ref{theorem:ulam}, the basic idea is to apply quantum amplitude estimation on the classical algorithm \textsf{UlamIndic} from Proposition~\ref{prop:Ulam}. Let us explain this strategy more precisely and show the technical difficulties we need to overcome. Assume that we know that $\edit(A,B)$ is in the interval $[D_1,D_2]$ for some values $D_1$ and $D_2$. We can then use  $\Estimator{A,B,\delta,t}$ with $t=c\cdot D_2$, and apply the quantum amplitude estimation algorithm of Theorem~\ref{th:ae} to estimate the probability it outputs~1. If we use~$k=\Theta(\sqrt{(n+t)/D_1})=\Theta(\sqrt{n/D_1})$  in Theorem~\ref{th:ae} and $\delta$ small enough, we will get a good approximation of the quantity $\edit(A,B)/(n+t)$, and thus a good approximation of $\edit(A,B)$. The complexity of this strategy is 
$
\tilde O(\sqrt{n/D_1}\cdot \sqrt{D_2}),
$
which is $\tilde O(\sqrt{n})$  when $D_1\approx D_2$. 

The main issue is that we do not know such tight upper and lower bounds on $\edit(A,B)$. Concerning the upper bound, we overcome this difficultly by simply successively trying $D_2=n$, $D_2=(1-\eta) n$, $D_2=(1-\eta)^2 n$, $\ldots$ for some small constant $\eta$. For the lower bound, on the other hand, we cannot simply start with $D_1=1$ and iteratively increase this value, since the cost would be too high: in order to achieve an overall running time of $\tilde O(\sqrt{n})$ we need to keep $D_1\approx D_2$. Instead of estimating the probability that \textsf{UlamIndic} outputs 1 using Theorem \ref{th:ae}, which is too costly, we thus design a gap test (see Proposition \ref{prop:qtest} below) that enables us to check if this probability is larger than $D_2$ or smaller than $(1-\eta)D_2$ much more efficiently, in time $\tilde O(\sqrt{n/D_2})$. 

We now present the details of our quantum algorithm. Let us first present the gap test.
This test relies on quantum amplitude amplification. Here is the precise statement of quantum amplitude amplification that we will use.

\begin{theorem}[Theorem 12 in \cite{brassard2002quantum}]\label{th:ae}
Let $\Aa$ be a classical algorithm that runs in time $T$, outputs~$1$ with probability $p$ and outputs $0$ with probability $1-p$, for some (unknown) value $p\in [0,1]$. For any integer $k\ge 1$, there exists a quantum algorithm that runs in time $\tilde O(kT)$ and outputs with probability at least $8/\pi^2$ an estimate $\tilde p$ such that
\[
|p-\tilde p|\le 2\pi\frac{\sqrt{p(1-p)}}{k}+\frac{\pi^2}{k^2}.
\]
\end{theorem}

The gap test is described in the following proposition.
\begin{proposition}\label{prop:qtest}
Let $\Aa$ be a classical algorithm that runs in time $T$, outputs~$1$ with probability $p$ and outputs $0$ with probability $1-p$, for some (unknown) value $p$.
For any $q\in(0,1]$ and any constant $\eta\in(0,1]$, there exists a quantum algorithm denoted $\Est{\Aa,q,\eta}$ that runs in time $\tilde O(T/\sqrt{q})$ and with probability at least $1-\poly(n)$ outputs \myLARGE{} if $p\ge q$ and \mySMALL{} if $p\le(1-\eta)q$.
\end{proposition}
\begin{proof}
Figure \ref{fig:qtest} describes our main quantum gap test. The complexity of this test is $\tilde O(T/\sqrt{q})$, from Theorem \ref{th:ae}. We show below that its success probability is at least $8/\pi^2$. The success probability can then be increased to $1-1/\poly(n)$ by repeating the test $\Theta(\log n)$ times and using majority voting.
\begin{figure}[h!]
\begin{center}
\fbox{
\begin{minipage}{14.5 cm} 
\begin{itemize}
\item[1.]
Apply the algorithm of Theorem \ref{th:ae} with 
$
k=\frac{20}{\eta\sqrt{q}}.
$
Let $\tilde p$ denote the output.
\item[2.]
Output \myLARGE{} if $\tilde p\ge (1-\eta/2)q$ and output \mySMALL{} if $\tilde p<(1-\eta/2)q$.
\end{itemize}
\end{minipage}
}
\end{center}
\vspace{-4mm}
\caption{Quantum gap test.}\label{fig:qtest}
\end{figure}

Let us analyze the success probability of the quantum gap test of Figure \ref{fig:qtest}. Note that Theorem~\ref{th:ae} guarantees that with probability at least $8/\pi^2$ the value $\tilde p$ satisfies the following two inequalities:
\begin{align}\label{ineq1}
\tilde p&\le p+2\pi\eta\frac{\sqrt{p(1-p)}\sqrt{q}}{20} + \pi^2\eta^2 \frac{q}{400},
\end{align}
\begin{align}\label{ineq2}
\tilde p&\ge p-2\pi\eta\frac{\sqrt{p(1-p)}\sqrt{q}}{20} - \pi^2\eta^2 \frac{q}{400}.
\end{align}

Let us first consider the case $p\le (1-\eta)q$. In that case Inequality (\ref{ineq1}) implies
\[
\tilde p \le (1-\eta)q+2\pi\eta \frac{q}{20}+\pi^2\eta^2\frac{q}{400}< (1-\eta/2)q
\]
since $2\pi/20+\pi^2/400<1/2$.
The probability that the algorithm outputs \myLARGE{} is thus at most $1-8/\pi^2$.

Now consider the case $p\ge q$. In that case Inequality (\ref{ineq2}) implies
\begin{align*}
\tilde p&\ge p-2\pi\eta\frac{\sqrt{p}\sqrt{q}}{20} - \pi^2\eta^2 \frac{q}{400}\\
&= \sqrt{p}\left(\sqrt{p}-2\pi\eta\frac{\sqrt{q}}{20}\right)- \pi^2\eta^2 \frac{q}{400}\\
&\ge q -2\pi \eta\frac{q}{20}-\pi^2\eta^2\frac{q}{400}> (1-\eta/2)q.
\end{align*}
The probability that the algorithm outputs \mySMALL{} is thus at most $1-8/\pi^2$.
\end{proof}


%on the algorithm from Proposition~\ref{prop:Ulam}
%If a good estimate $D$ of $\edit(A,B)$ were known, 
%Using Theorem \ref{th:ae}, this would require applying Algorithm $\Estimator{}$ about $\sqrt{n/\edit(A,B)}$ times.

% in order to construct a $\tilde O(\sqrt{n})$-time quantum algorithm that gives a $(1+\epsilon)$-approximation of $\edit(A,B)$.
%\Francois{It would be nice to add a more detailed informal description of the algorithm.}

We are now ready to give the proof of Theorem \ref{theorem:ulam}.
\begin{proof}[Proof of Theorem \ref{theorem:ulam}]
If $\edit(A,B)\ge \sqrt{n}$ then $\edit(A,B)$ can already be computed in $\tilde O(\sqrt{n})$ time by the classical algorithm from \cite{Naumovitz+SODA17}. We thus assume below that $\edit(A,B)\le \sqrt{n}$. We also assume that $\edit(A,B)>0$, since otherwise the two strings are identical, which can be checked in $\tilde O(\sqrt{n})$ time using Grover search.

Below we will invoke Algorithm $\Estimator{A,B,\delta,t}$ with values of $t$ such that $t\le \sqrt{n}$. Let us call $p_t$ the probability that it outputs $1$. Note that Proposition \ref{prop:Ulam} guarantees that
\begin{equation}\label{rel}
p_t\in \left[(1-\delta)\left(1-\frac{1}{\sqrt{n}}\right)\cdot \frac{\edit(A,B)}{n},(1+\delta)\cdot \frac{\edit(A,B)}{n}+\frac{\delta}{n}\right]
\end{equation}
for any $t\le \sqrt{n}$.

Our quantum algorithm is described in Figure \ref{fig:qalg}.

%Let us fix $\eta=\Theta(\epsilon)$.  We describe the quantum algorithm below.
\begin{figure}[h!]
\begin{center}
\fbox{
\begin{minipage}{13 cm} 
\begin{itemize}
\item[1.]
Set $\eta=\epsilon/10$ and $\delta=\epsilon/3$ and $r=\ceil{\frac{\log((1-\delta)(\sqrt{n}-1)/n)}{\log (1-\eta)}}$. 
\item[2.] 
For i from $1$ to $r$ do:
\begin{itemize}
\item[2.1.]
Set $q=(1-\eta)^i /\sqrt{n}$ and $t=(1-\eta)^i \sqrt{n}$.
\item[2.2.]
Apply Algorithm $\Est{\Aa,q,\eta}$ with $\Aa=\Estimator{A,B,\delta,t}$. \Saeed{Comment from the reviewers: Figure 13, 2.2. The guarantee of proposition 2 holds under the assumption that $t>c\cdot ud(A,b)$. Using the exact values of $t$ given, this may not be the case depending on $c$, though a constant factor on $t$ when calling UlamIndic should solve this issue.}
\item[2.3.]
If the output is \myLARGE{}, then stop and return $t$.
\end{itemize}
\item[3.]
Return \Error{}.
\end{itemize}
\end{minipage}
}
\end{center}
\vspace{-2mm}
\caption{Quantum algorithm computing a $(1+\epsilon)$-approximation of the Ulam distance of two strings $A$ and $B$.}\label{fig:qalg}
\end{figure}

First observe that for $r=\ceil{\frac{\log((1-\delta)(\sqrt{n}-1)/n)}{\log (1-\eta)}}$, the inequality 
\[
(1-\delta)\left(1-\frac{1}{\sqrt{n}}\right)\cdot \frac{\edit(A,B)}{n}\ge (1-\eta)^r/\sqrt{n}
\]
holds, since we are assuming that $\edit(A,B)\ge 1$.
From Proposition \ref{prop:qtest} combined with (\ref{rel}), this means that with probability at least $1-1/\poly(n)$, the algorithm will never reach Step $3$ (and thus does not output \Error{}). In the remaining of the proof, we assume that the algorithm stops before reaching Step 3. Let~$i^\ast$ denote the value of $i$ during the last iteration of the loop of Step 2, and write $q^\ast=(1-\eta)^{i^\ast}/\sqrt{n}$ and $t^\ast=(1-\eta)^{i^\ast}\sqrt{n}$. Observe that the output of the algorithm is $t^\ast$. 

Assume first that $i^\ast=1$. The output is thus $t^\ast=(1-\eta)\sqrt{n}$. Observe that Algorithm $\textsf{QTest}$ then necessarily outputted $\myLARGE$ for $i=1$. Proposition \ref{prop:qtest} guarantees that with probability at least $1-1/\poly(n)$ the inequality $p_{t^\ast}\ge (1-\eta)q^\ast$ holds (otherwise it would have outputted $\mySMALL$). 
This inequality combined with (\ref{rel}) implies that
\[
(1+\delta)\cdot \frac{\edit(A,B)}{n}+\frac{\delta}{n}\ge (1-\eta)q^\ast
\]
and thus the output $t^\ast=nq^\ast$ of the algorithm satisfies the following inequalities:
\begin{align}\label{ineq:UB}
\begin{aligned}
t^\ast&\le ((1+\delta)\cdot \edit(A,B)+\delta)/(1-\eta)\\
&\le (1+2\delta)\cdot\edit(A,B)/ (1-\eta)\\
&\le (1+2\delta)(1+2\eta) \cdot \edit(A,B)\\
&\le (1+\epsilon) \cdot \edit(A,B),
\end{aligned}
\end{align}
where we used the inequality $1/(1-x)\le 1+2x$, which holds for any $x\in[0,1/2]$. Also note that the inequality 
\[
t^\ast\ge (1-\epsilon)\cdot\edit(A,B)
\]
is trivially satisfied since we are assuming $\edit(A,B)\le \sqrt{n}$ and $\eta<\epsilon$.
The output is thus a $(1+\epsilon)$-approximation of $\edit(A,B)$.

Assume now that $i^\ast\ge 2$. 
%\Francois{We also need to consider $i^\ast=1$, but this ``degenerate’’ case is actually easier since we can use the trivial upper bound $\edit(A,B)\le \sqrt{n}$.} 
Observe that Algorithm $\textsf{QTest}$ then necessarily outputted $\myLARGE$ for $i=i^\ast$ and $\mySMALL$ for $i= i^\ast-1$. 
Since it outputted $\myLARGE$ for $i=i^\ast$, Inequalities (\ref{ineq:UB}) hold with probability at least $1-1/\poly(n)$, from exactly the same argument as above. Since the output was $\mySMALL$ for $i=i^\ast-1$, Proposition \ref{prop:qtest} guarantees that with probability at least $1-1/\poly(n)$ the inequality
$
p_{t^\ast/(1-\eta)}\le q^\ast/(1-\eta)
$
holds (otherwise it would have outputted $\myLARGE$).
%\Francois{Maybe add some explanations about why the output of $\textsf{QTest}$ for $i=i^\ast-1$ cannot be directly used (this is because the output of \textsf{QTest} may be wrong near the threshold, so we need a gap to make a correct decision).}
Since $t^\ast=nq^\ast$, this inequality combined with (\ref{rel}) implies:
\begin{align*}
t^\ast&\ge n(1-\eta)p_{t^\ast/(1-\eta)}\\
&\ge (1-\eta)(1-\delta)\left(1-\frac{1}{\sqrt{n}}\right)\cdot \edit(A,B)\\
&= (1-\epsilon/10)(1-\epsilon/3)\left(1-\frac{1}{\sqrt{n}}\right)\cdot \edit(A,B)\\
&\ge (1-\epsilon)\cdot \edit(A,B).
\end{align*}
%where we used the inequality $1/(1-x)\le 1+2x$, which holds for any $x\in[0,1/2]$, to derive the last line.
\Francois{May need to adjust a bit the values of $\eta$ and $\delta$.}
The output of the algorithm is thus a $(1+\epsilon)$-approximation of $\edit(A,B)$ as well. 

Since the complexity of applying Algorithm \textsf{UlamIndic} at Step $i$ is $\tilde O(\sqrt{(1-\eta)^i\sqrt{n}})$, the
overall complexity of the algorithm is 
\[
\tilde O\left(\sum_{i=1}^{r} \frac{1}{\sqrt{(1-\eta)^i/\sqrt{n}}}\sqrt{(1-\eta)^i\sqrt{n}}\right)
=
\tilde O\left(\sqrt{n}\right),
\]
as claimed.
\end{proof}

==> src/old files/ulam-distance.tex <==


\section{Constant-factor Approximation of the Ulam Distance}
Andoni and Nguyen \cite{Andoni+SODA10} have given a classical algorithm that computes a constant-factor approximation of the edit distance of two non-repetitive strings in time $\tilde O(n/\ell+\sqrt{n})$, where $n$ is the length of the strings and $\ell$ is their edit distance. Here is our conjecture. \Saeed{I use $d$ for the size of the solution, can you replace $\ell$ with $d$ so that we are consistent throughout the paper?} 

\begin{conjecture}
There is a quantum algorithm that computes with high probability a constant-factor approximation of the edit distance of two non-repetitive strings in time $\tilde O(\sqrt{n/\ell}+n^{1/3})$.
\end{conjecture}
The following is a simple consequence of this conjecture.

\begin{theorem}\label{th:main}
There is a quantum algorithm that computes with high probability a constant-factor approximation of the edit distance of two non-repetitive strings in time $\tilde O(\sqrt{n})$.
\end{theorem}

In this note we will give an overview of the proof of Theorem \ref{th:main}. Since the classical algorithm from \cite{Andoni+SODA10} has already complexity $\tilde O(\sqrt{n})$ when $\ell\ge \sqrt{n}$, our goal will be to construct a quantum algorithm with running time $\tilde O(\sqrt{n})$ for the case $\ell\le \sqrt{n}$.

%=========================================
\subsection{Overview of the Classical Algorithm}
%=========================================
Let $A$ and $B$ denote the two input strings. The main algorithm from \cite{Andoni+SODA10} that we will use to build our quantum algorithm is the following result. \Saeed{Can you bring more discussion about the AN algorithm? Things like they design 3 gap tests, slow, medium, and fast and how they use them to obtain the solution.}
\begin{lemma}[Lemma 4.1 in \cite{Andoni+SODA10}]
For any $a$, there is a $\tilde O(n/\sqrt{a})$-time classical algorithm that distinguishes between the case $\edit(A,B)<a$ and the case $\edit(A,B)>512a$.
\end{lemma}
\Saeed{The above is the medium gap-test, right? What about the slow and the fast one?}

In the remaining of the section we will describe this classical algorithm. For any substrings $A[i_A,\ldots,j_A]$ and $B[i_B\ldots,j_B]$, we define the quantity $\Nn_a(A[i_A,\ldots,j_A],B[i_B\ldots,j_B])$ as the number of pairs $(u,v)\in [i_A,\ldots,j_A]\times [i_B,\ldots,j_B]$ such that $A[u]=B[v]$ and 
\begin{equation}\label{eq:0}
|A[u-z,u-1]\Delta B[v-z,v-1]|>z \:\textrm{ holds for some } z<4a.
\end{equation} 
\Saeed{I'm having a bit of difficulty understanding the above definition. Can you bring more intuition to make it simpler to understand? Perhaps an example?}
We first divide $A$ and $B$ into $n/a$ blocks of size $a$. Let us write $s=n/a$ and write $A_1,\ldots,A_{s}$ and $B_1,\ldots,B_{s}$ these blocks. For each $i\in[0,\log a]$, let $\hat{X}_i$ be \mycomment{a good approximation of}\footnote{In this memo I don't give a precise definition of the precision needed in the approximations of the terms written in red.} the number of indices $k\in[1,s-2]$ such that
\begin{equation}\label{eq:T1}
\Big|
A[ka+1,(k+1)a]\setminus B[(k-1)a+1,(k+2)a]
\Big|
\mycomment{\approx} \:
2^i.
\end{equation}
For each $i\in[0,\log a]$, let $\hat{Y}_i$ be \mycomment{a good approximation of} the number of indices $k\in[1,s-2]$ such that
\begin{equation}\label{eq:T2}
\Big|\Nn_a(A[ka+1,(k+1)a],B[(k-1)a+1,(k+2)a])\big|
\mycomment{\approx} \:
2^i.
\end{equation}
Define 
\[
\hat X=\sum_{i=0}^a \hat{X}_i 2^i\:\:\: \textrm{ and }\:\:\:
\hat{Y}=\sum_{i=0}^a \hat{Y}_i 2^i.
\]
The analysis done in \cite{Andoni+SODA10} shows the following:
\begin{itemize}
\item If $\edit(A,B)<a$ then $\hat{X}+\hat{Y}<a/10$,
\item If $\edit(A,B)>512a$ then $\hat{X}+\hat{Y}>a/10$.
\end{itemize}
The intuition is as follows. The term $\hat X$ counts the character movements between different blocks. Term $\hat Y$ counts the character movements within each blocks, which is characterized as the number of characters witnessing a lot of inversion in their neighborhood.

For a fixed $(i,k)$, Andoni and Nguyen show how to check if Equation (\ref{eq:T1}) holds in time 
\[
\tilde O\left(
%\min\left(a,
\frac{a\sqrt{a}}{2^i}
%\right)
\right).
\]
%Note that the first term is trivial: just read all the characters in $A[ka+1,(k+1)a]$ and $B[(k-1)a+1,(k+2)a]$. 
This is done by randomly sampling $a\sqrt{a}/2^i$ characters of each $A[ka+1,(k+1)a]$ and $B[(k-1)a+1,(k+2)a]$, computing the number of collisions $C$ among the sampled characters, and then testing if 
\[
a-\frac{2^{2i}}{a}\cdot C \:\mycomment{\approx}\: 2^i.
\]

For a fixed $(i,k)$, Andoni and Nguyen show how to check if Equation (\ref{eq:T2}) holds in time 
\[
\tilde O\left(\frac{a}{2^{i/2}}+ \frac{a\sqrt{a}}{2^i}\right).
\]
This is done by randomly sampling $a/2^{i/2}$ characters of each $A[ka+1,(k+1)a]$ and $B[(k-1)a+1,(k+2)a]$, finding all the collisions $A[u]=B[v]$ and for each such collision checking if Equation (\ref{eq:0}) holds using a $O(\sqrt{a})$-time procedure called YContributingTest (which is again based on collision finding). The above complexity comes from the observation that there are about $a/2^{i}$ collisions.

The whole complexity of the classical algorithm is:
\[
\tilde O\left(
\sum_{i=0}^{\log a}\mycomment{\frac{2^i n}{a^2}}\left(
%\min\left(a,
\frac{a\sqrt{a}}{2^i}
%\right)
+
\frac{a}{2^{i/2}}+ \frac{a\sqrt{a}}{2^i}
\right)\right)=
\tilde O(n/\sqrt{a}),
\]
as claimed. The red term comes from the observation that for each $i$, there can only be at most $a/2^i$ indices $k$ contributing to $\hat{X}_i$ (and similarly for $\hat{Y}_i$) so a good approximation of  $\hat{X}_i$ and $\hat{Y}_i$ can be obtained by sampling $\frac{n/a}{a/2^i}=\frac{n2^i}{a^2}$ indices $k$ uniformly at random. 

%==============================
\subsection{Quantum algorithm}
%==============================
%We will need the following lemma about amplitude amplification.
%\begin{lemma}[Theorem 6 in \cite{Brassard+98}]\label{amp}
%Consider a quantum process $\Qq$ that outputs ``accept'' with some unknown probability $p$. For any $\delta>0$, an estimator $\tilde p$ such that $|\tilde p - p|\le \delta p$ can be computed using $O(\frac{1}{\delta \sqrt{p}})$ calls to $\Qq$.
%\end{lemma}

We show the following propositions.
\begin{proposition}
Given $(k,i)$, we can check if Equation (\ref{eq:T1}) holds in time 
\[
\tilde O\left(\blue{\frac{a}{2^{i/2}}}\right)
\] 
using a quantum algorithm.
\end{proposition}
\begin{proof}
We count the number of characters in $A[ka+1,(k+1)a]$ that are not in $B[(k-1)a+1,(k+2)a]$ in order to check whether Equation (\ref{eq:T1}) holds. Using approximate counting \cite{Brassard+98}, this can be done in time 
\[
\tilde O\left(\sqrt{\frac{a}{2^i}}\sqrt{a}\right)=\tilde O\left(\frac{a}{2^{i/2}}\right).
\]
\end{proof}
%\begin{proposition}
%Given $(k,i)$, we can check if Equation (\ref{eq:T1}) holds in time 
%\[
%\tilde O\left(\frac{a}{2^{2i/3}}\right)
%\] 
%using a quantum algorithm.
%\end{proposition}
%\begin{proof}
%Note that Equation (\ref{eq:T1}) holds if and only if the number of collisions between $A[ka+1,(k+1)a]$ and $B[(k-1)a+1,(k+2)a]$, which we write $C$ below, is \red{close to} $a-2^i$.
%
%Let us consider a quantum-walk approach similar to \cite{AmbainisSICOMP07,Magniez+SICOMP11} for finding one of such collisions. This approach can be described as follows. For some parameter $r$, we perform a setup operation that costs $O(r)$ queries and then we apply $O(\sqrt{a^2/(Cr^2)})$ times the following quantum process:
%\begin{itemize}
%\item[1.]
%implement $\Theta(\sqrt{r})$ steps of a quantum walk over the Johnson graph corresponding to $r$-subsets of the search space;
%\item[2.]
%check if we have a solution.
%\end{itemize}
%The overal complexity is 
%\[
%\tilde O\left(r + \sqrt{\frac{a^2}{Cr^2}}(\sqrt{r}\times 1 + 0)\right).
%\]
%
%Let us write $p=Cr^2/a^2$.
%By using amplitude estimation (Lemma \ref{amp}), instead of amplitude amplification, I believe that we can obtain an estimator $\tilde p$ such that $|p-\tilde p|<\delta p$ in time
%\[
%\tilde O\left(r + \frac{1}{\delta}\sqrt{\frac{a^2}{Cr^2}}(\sqrt{r}\times 1 + 0)\right).
%\]
%By taking $\delta = \Theta(2^i/C)$ and outputting $\tilde pa^2/r^2$, we obtain a $2^i$-additive approximation of $C$ with high probability. The complexity of this approach is 
%\[
%\tilde O\left(r + \frac{C}{2^i}\sqrt{\frac{a^2}{Cr^2}}(\sqrt{r}\times 1 + 0)\right)=
%\tilde O\left(r + \frac{a^{3/2}}{2^i\sqrt{r}}\right).
%\]
%This expression is minimized for $r=a/2^{2i/3}$, which gives the claimed complexity.
%\end{proof}
\begin{proposition}
Given $(k,i)$, we can check if Equation (\ref{eq:T2}) holds in time 
\[
\tilde O\left(\blue{\frac{a}{2^{i/2}}}+ \frac{a^{5/6}}{2^{i/2}}\right)
\] 
using a quantum algorithm. 
\end{proposition}
\begin{proof}
We first take $a/2^{i/2}$ characters of each $A[ka+1,(k+1)a]$ and $B[(k-1)a+1,(k+2)a]$, as in the classical setting. There are about $a/2^{i}$ collisions, and we want to decide if there exists a constant number of such collisions that satisfy Equation (\ref{eq:0}). Testing if a collision satisfies this equation can be done in time $O(a^{1/3})$ by modifying the classical procedure YContributingTest.\footnote{The classical procedure outputs a constant-factor approximation of the number of collisions, which can be done in time $\tilde O(\sqrt{a})$ classically. In the quantum setting, we can use quantum walks (see \cite{AmbainisSICOMP07}) to do this in time $\tilde O(a^{1/3})$.} The overall complexity is thus
\[
\tilde O\left(\frac{a}{2^{i/2}} + \sqrt{\frac{a}{2^{i}}}a^{1/3}\right)=\tilde O\left(\frac{a}{2^{i/2}}+ \frac{a^{5/6}}{2^{i/2}}\right).
\] 
\end{proof}

By using additionally quantum approximate counting \cite{Brassard+98} for the red term below, we get overall complexity 
\[
\tilde O\left(
\sum_{i=0}^{\log a}\mycomment{\sqrt{\frac{2^i n}{a^2}}}\left(
\blue{\frac{a}{2^{i/2}}}+
\blue{\frac{a}{2^{i/2}}}+ \frac{a^{5/6}}{2^{i/2}}
\right)\right)=
\tilde O(\sqrt{n}).
\]

\noindent {\bf Remark.}
The blue terms can probably be improved, so that the overall complexity of the quantum algorithm will probably become $\tilde O(\sqrt{n}/a^{1/6})$.
%=====================================
%=====================================


